The Role of Memory in Stochastic Optimization

The choice of how to retain information about past gradients dramatically affects the convergence properties of state-of-the-art stochastic optimization methods, such as Heavy-ball, Nesterov's momentum, RMSprop and Adam. Building on this observation, we use stochastic differential equations (SDEs) to explicitly study the role of memory in gradient-based algorithms. We first derive a general continuous-time model that can incorporate arbitrary types of memory, for both deterministic and stochastic settings. We provide convergence guarantees for this SDE for weakly-quasi-convex and quadratically growing functions. We then demonstrate how to discretize this SDE to get a flexible discrete-time algorithm that can implement a board spectrum of memories ranging from short- to long-term. Not only does this algorithm increase the degrees of freedom in algorithmic choice for practitioners but it also comes with better stability properties than classical momentum in the convex stochastic setting. In particular, no iterate averaging is needed for convergence. Interestingly, our analysis also provides a novel interpretation of Nesterov's momentum as stable gradient amplification and highlights a possible reason for its unstable behavior in the (convex) stochastic setting. Furthermore, we discuss the use of long term memory for second-moment estimation in adaptive methods, such as Adam and RMSprop. Finally, we provide an extensive experimental study of the effect of different types of memory in both convex and nonconvex settings.

==> algorithm.tex <==
% ALGORITHM STYLE -- Released 8 April 1996
%    for LaTeX-2e
% Copyright -- 1994 Peter Williams
% E-mail Peter.Williams@dsto.defence.gov.au
\NeedsTeXFormat{LaTeX2e}
\ProvidesPackage{algorithm}
\typeout{Document Style `algorithm' - floating environment}

\RequirePackage{float}
\RequirePackage{ifthen}
\newcommand{\ALG@within}{nothing}
\newboolean{ALG@within}
\setboolean{ALG@within}{false}
\newcommand{\ALG@floatstyle}{ruled}
\newcommand{\ALG@name}{Algorithm}
\newcommand{\listalgorithmname}{List of \ALG@name s}

% Declare Options
% first appearance
\DeclareOption{plain}{
  \renewcommand{\ALG@floatstyle}{plain}
}
\DeclareOption{ruled}{
  \renewcommand{\ALG@floatstyle}{ruled}
}
\DeclareOption{boxed}{
  \renewcommand{\ALG@floatstyle}{boxed}
}
% then numbering convention
\DeclareOption{part}{
  \renewcommand{\ALG@within}{part}
  \setboolean{ALG@within}{true}
}
\DeclareOption{chapter}{
  \renewcommand{\ALG@within}{chapter}
  \setboolean{ALG@within}{true}
}
\DeclareOption{section}{
  \renewcommand{\ALG@within}{section}
  \setboolean{ALG@within}{true}
}
\DeclareOption{subsection}{
  \renewcommand{\ALG@within}{subsection}
  \setboolean{ALG@within}{true}
}
\DeclareOption{subsubsection}{
  \renewcommand{\ALG@within}{subsubsection}
  \setboolean{ALG@within}{true}
}
\DeclareOption{nothing}{
  \renewcommand{\ALG@within}{nothing}
  \setboolean{ALG@within}{true}
}
\DeclareOption*{\edef\ALG@name{\CurrentOption}}

% ALGORITHM
%
\ProcessOptions
\floatstyle{\ALG@floatstyle}
\ifthenelse{\boolean{ALG@within}}{
  \ifthenelse{\equal{\ALG@within}{part}}
     {\newfloat{algorithm}{htbp}{loa}[part]}{}
  \ifthenelse{\equal{\ALG@within}{chapter}}
     {\newfloat{algorithm}{htbp}{loa}[chapter]}{}
  \ifthenelse{\equal{\ALG@within}{section}}
     {\newfloat{algorithm}{htbp}{loa}[section]}{}
  \ifthenelse{\equal{\ALG@within}{subsection}}
     {\newfloat{algorithm}{htbp}{loa}[subsection]}{}
  \ifthenelse{\equal{\ALG@within}{subsubsection}}
     {\newfloat{algorithm}{htbp}{loa}[subsubsection]}{}
  \ifthenelse{\equal{\ALG@within}{nothing}}
     {\newfloat{algorithm}{htbp}{loa}}{}
}{
  \newfloat{algorithm}{htbp}{loa}
}
\floatname{algorithm}{\ALG@name}

\newcommand{\listofalgorithms}{\listof{algorithm}{\listalgorithmname}}



==> algorithmic.tex <==
% ALGORITHMIC STYLE -- Released 8 APRIL 1996
%    for LaTeX version 2e
% Copyright -- 1994 Peter Williams
% E-mail PeterWilliams@dsto.defence.gov.au
%
% Modified by Alex Smola (08/2000)
% E-mail Alex.Smola@anu.edu.au
%
\NeedsTeXFormat{LaTeX2e}
\ProvidesPackage{algorithmic}
\typeout{Document Style `algorithmic' - environment}
%
\RequirePackage{ifthen}
\RequirePackage{calc}
\newboolean{ALC@noend}
\setboolean{ALC@noend}{false}
\newcounter{ALC@line}
\newcounter{ALC@rem}
\newlength{\ALC@tlm}
%
\DeclareOption{noend}{\setboolean{ALC@noend}{true}}
%
\ProcessOptions
%
% ALGORITHMIC
\newcommand{\algorithmicrequire}{\textbf{Require:}}
\newcommand{\algorithmicensure}{\textbf{Ensure:}}
\newcommand{\algorithmiccomment}[1]{\{#1\}}
\newcommand{\algorithmicend}{\textbf{end}}
\newcommand{\algorithmicif}{\textbf{if}}
\newcommand{\algorithmicthen}{\textbf{then}}
\newcommand{\algorithmicelse}{\textbf{else}}
\newcommand{\algorithmicelsif}{\algorithmicelse\ \algorithmicif}
\newcommand{\algorithmicendif}{\algorithmicend\ \algorithmicif}
\newcommand{\algorithmicfor}{\textbf{for}}
\newcommand{\algorithmicforall}{\textbf{for all}}
\newcommand{\algorithmicdo}{\textbf{do}}
\newcommand{\algorithmicendfor}{\algorithmicend\ \algorithmicfor}
\newcommand{\algorithmicwhile}{\textbf{while}}
\newcommand{\algorithmicendwhile}{\algorithmicend\ \algorithmicwhile}
\newcommand{\algorithmicloop}{\textbf{loop}}
\newcommand{\algorithmicendloop}{\algorithmicend\ \algorithmicloop}
\newcommand{\algorithmicrepeat}{\textbf{repeat}}
\newcommand{\algorithmicuntil}{\textbf{until}}

%changed by alex smola
\newcommand{\algorithmicinput}{\textbf{input}}
\newcommand{\algorithmicoutput}{\textbf{output}}
\newcommand{\algorithmicset}{\textbf{set}}
\newcommand{\algorithmictrue}{\textbf{true}}
\newcommand{\algorithmicfalse}{\textbf{false}}
\newcommand{\algorithmicand}{\textbf{and\ }}
\newcommand{\algorithmicor}{\textbf{or\ }}
\newcommand{\algorithmicfunction}{\textbf{function}}
\newcommand{\algorithmicendfunction}{\algorithmicend\ \algorithmicfunction}
\newcommand{\algorithmicmain}{\textbf{main}}
\newcommand{\algorithmicendmain}{\algorithmicend\ \algorithmicmain}
%end changed by alex smola

\def\ALC@item[#1]{%
\if@noparitem \@donoparitem
  \else \if@inlabel \indent \par \fi
         \ifhmode \unskip\unskip \par \fi
         \if@newlist \if@nobreak \@nbitem \else
                        \addpenalty\@beginparpenalty
                        \addvspace\@topsep \addvspace{-\parskip}\fi
           \else \addpenalty\@itempenalty \addvspace\itemsep
          \fi
    \global\@inlabeltrue
\fi
\everypar{\global\@minipagefalse\global\@newlistfalse
          \if@inlabel\global\@inlabelfalse \hskip -\parindent \box\@labels
             \penalty\z@ \fi
          \everypar{}}\global\@nobreakfalse
\if@noitemarg \@noitemargfalse \if@nmbrlist \refstepcounter{\@listctr}\fi \fi
\sbox\@tempboxa{\makelabel{#1}}%
\global\setbox\@labels
 \hbox{\unhbox\@labels \hskip \itemindent
       \hskip -\labelwidth \hskip -\ALC@tlm
       \ifdim \wd\@tempboxa >\labelwidth
                \box\@tempboxa
          \else \hbox to\labelwidth {\unhbox\@tempboxa}\fi
       \hskip \ALC@tlm}\ignorespaces}
%
\newenvironment{algorithmic}[1][0]{
\let\@item\ALC@item
  \newcommand{\ALC@lno}{%
\ifthenelse{\equal{\arabic{ALC@rem}}{0}}
{{\footnotesize \arabic{ALC@line}:}}{}%
}
\let\@listii\@listi
\let\@listiii\@listi
\let\@listiv\@listi
\let\@listv\@listi
\let\@listvi\@listi
\let\@listvii\@listi
  \newenvironment{ALC@g}{
    \begin{list}{\ALC@lno}{ \itemsep\z@ \itemindent\z@
    \listparindent\z@ \rightmargin\z@ 
    \topsep\z@ \partopsep\z@ \parskip\z@\parsep\z@
    \leftmargin 1em
    \addtolength{\ALC@tlm}{\leftmargin}
    }
  }
  {\end{list}}
  \newcommand{\ALC@it}{\addtocounter{ALC@line}{1}\addtocounter{ALC@rem}{1}\ifthenelse{\equal{\arabic{ALC@rem}}{#1}}{\setcounter{ALC@rem}{0}}{}\item}
  \newcommand{\ALC@com}[1]{\ifthenelse{\equal{##1}{default}}%
{}{\ \algorithmiccomment{##1}}}
  \newcommand{\REQUIRE}{\item[\algorithmicrequire]}
  \newcommand{\ENSURE}{\item[\algorithmicensure]}
  \newcommand{\STATE}{\ALC@it}
  \newcommand{\COMMENT}[1]{\algorithmiccomment{##1}}
%changes by alex smola
  \newcommand{\INPUT}{\item[\algorithmicinput]}
  \newcommand{\OUTPUT}{\item[\algorithmicoutput]}
  \newcommand{\SET}{\item[\algorithmicset]}
%  \newcommand{\TRUE}{\algorithmictrue}
%  \newcommand{\FALSE}{\algorithmicfalse}
  \newcommand{\AND}{\algorithmicand}
  \newcommand{\OR}{\algorithmicor}
  \newenvironment{ALC@func}{\begin{ALC@g}}{\end{ALC@g}}
  \newenvironment{ALC@main}{\begin{ALC@g}}{\end{ALC@g}}
%end changes by alex smola
  \newenvironment{ALC@if}{\begin{ALC@g}}{\end{ALC@g}}
  \newenvironment{ALC@for}{\begin{ALC@g}}{\end{ALC@g}}
  \newenvironment{ALC@whl}{\begin{ALC@g}}{\end{ALC@g}}
  \newenvironment{ALC@loop}{\begin{ALC@g}}{\end{ALC@g}}
  \newenvironment{ALC@rpt}{\begin{ALC@g}}{\end{ALC@g}}
  \renewcommand{\\}{\@centercr}
  \newcommand{\IF}[2][default]{\ALC@it\algorithmicif\ ##2\ \algorithmicthen%
\ALC@com{##1}\begin{ALC@if}}
  \newcommand{\SHORTIF}[2]{\ALC@it\algorithmicif\ ##1\
    \algorithmicthen\ {##2}}
  \newcommand{\ELSE}[1][default]{\end{ALC@if}\ALC@it\algorithmicelse%
\ALC@com{##1}\begin{ALC@if}}
  \newcommand{\ELSIF}[2][default]%
{\end{ALC@if}\ALC@it\algorithmicelsif\ ##2\ \algorithmicthen%
\ALC@com{##1}\begin{ALC@if}}
  \newcommand{\FOR}[2][default]{\ALC@it\algorithmicfor\ ##2\ \algorithmicdo%
\ALC@com{##1}\begin{ALC@for}}
  \newcommand{\FORALL}[2][default]{\ALC@it\algorithmicforall\ ##2\ %
\algorithmicdo%
\ALC@com{##1}\begin{ALC@for}}
  \newcommand{\SHORTFORALL}[2]{\ALC@it\algorithmicforall\ ##1\ %
    \algorithmicdo\ {##2}}
  \newcommand{\WHILE}[2][default]{\ALC@it\algorithmicwhile\ ##2\ %
\algorithmicdo%
\ALC@com{##1}\begin{ALC@whl}}
  \newcommand{\LOOP}[1][default]{\ALC@it\algorithmicloop%
\ALC@com{##1}\begin{ALC@loop}}
%changed by alex smola
  \newcommand{\FUNCTION}[2][default]{\ALC@it\algorithmicfunction\ ##2\ %
    \ALC@com{##1}\begin{ALC@func}}
  \newcommand{\MAIN}[2][default]{\ALC@it\algorithmicmain\ ##2\ %
    \ALC@com{##1}\begin{ALC@main}}
%end changed by alex smola
  \newcommand{\REPEAT}[1][default]{\ALC@it\algorithmicrepeat%
    \ALC@com{##1}\begin{ALC@rpt}}
    \newcommand{\UNTIL}[1]{\end{ALC@rpt}\ALC@it\algorithmicuntil\ ##1}
  \ifthenelse{\boolean{ALC@noend}}{
    \newcommand{\ENDIF}{\end{ALC@if}}
    \newcommand{\ENDFOR}{\end{ALC@for}}
    \newcommand{\ENDWHILE}{\end{ALC@whl}}
    \newcommand{\ENDLOOP}{\end{ALC@loop}}
    \newcommand{\ENDFUNCTION}{\end{ALC@func}}
    \newcommand{\ENDMAIN}{\end{ALC@main}}
  }{
    \newcommand{\ENDIF}{\end{ALC@if}\ALC@it\algorithmicendif}
    \newcommand{\ENDFOR}{\end{ALC@for}\ALC@it\algorithmicendfor}
    \newcommand{\ENDWHILE}{\end{ALC@whl}\ALC@it\algorithmicendwhile}
    \newcommand{\ENDLOOP}{\end{ALC@loop}\ALC@it\algorithmicendloop}
    \newcommand{\ENDFUNCTION}{\end{ALC@func}\ALC@it\algorithmicendfunction}
    \newcommand{\ENDMAIN}{\end{ALC@main}\ALC@it\algorithmicendmain}
  } 
  \renewcommand{\@toodeep}{}
  \begin{list}{\ALC@lno}{\setcounter{ALC@line}{0}\setcounter{ALC@rem}{0}%
      \itemsep\z@ \itemindent\z@ \listparindent\z@%
      \partopsep\z@ \parskip\z@ \parsep\z@%
      \labelsep 0.5em \topsep 0.2em%
      \ifthenelse{\equal{#1}{0}}
      {\labelwidth 0.5em }
      {\labelwidth  1.2em }
      \leftmargin\labelwidth \addtolength{\leftmargin}{\labelsep}
      \ALC@tlm\labelsep
      }
    }
  {\end{list}}
















==> sections/old/OLD_background.tex <==
\section{Memory perspective on HB}
\label{sec:background}

We provide an alternative view on momentum methods which builds on top of the theoretical work on memory gradient diffusion developed by~\cite{cabot2009long, gadat2014long}. First, we rewrite \ref{HB} (initialized with $x_0=x_{-1}$) as
\begin{tcolorbox}
\begin{equation}
\tag{HB-SUM}
\hspace{-1mm}
x_{k+1} = x_k - \eta \sum_{j=0}^{k-1} \left(\prod_{h=j+1}^k\beta_h\right) \nabla f(x_j)- \eta\nabla f(x_k)
\label{HB-SUM}
\end{equation}
\end{tcolorbox}
that is, at iteration $k$ we decide the next step using a weighted average of past gradients: in particular, if $\beta_i$ is constant, the memory vanishes exponentially fast. Such averaging provides a cheap way to 1) adapt to the geometry of ill-conditioned problems (also noted in \cite{sutskever13}) and 2) denoise stochastic gradients if the underlying true gradients are changing slowly. The latter observation led to the introduction of the bias-correction term in ADAM \cite{kingma2014adam}; we remind the reasoning behind it in the next few lines.

In the limit case where true gradients are constant, the averaging procedure in \ref{HB-SUM} is biased: let $i_j\in[N]$ be the data-point selected at iteration $j$ and $\nabla f_{i_j}$ the corresponding stochastic gradient; if we define $\epsilon_j:= \nabla f(x_j)-\nabla f_{i_j}(x_j)$ and pick constant momentum $\beta_j = \beta$, we have
\begin{align*}
    \E\left[\sum_{j=0}^{k} \beta^{k-j} \nabla f_{i_j}(x_j)\right] &= \sum_{j=0}^{k} \beta^{k-j} \E[\nabla f + \epsilon_j]\\
    &= \frac{\beta^{k+1}-1}{\beta -1} \nabla f. 
\end{align*}
Therefore ---to ensure an unbiased update, at least for this simple case--- \cite{kingma2014adam} normalize the sum above  by $\frac{\beta^{k+1}-1}{\beta -1}$, showing significant benefits in the experimental section. Indeed, such normalization retains all the celebrated geometric properties of momentum, while improving statistical accuracy  ---a crucial feature of SGD. In addition, we show in Appendix~\ref{sec:app_background} that such normalization also performs variance reduction.

Therefore, supported by the empirical success of ADAM, it seems reasonable to modify standard Heavy Ball (Eq.~\ref{HB-SUM}) with constant momentum to match the ADAM update:
 \begin{equation}
    x_{k+1} = x_k - \eta \frac{\beta-1}{\beta^{k+1}-1} \sum_{j=0}^{k} \beta^{k-j} \nabla f(x_j).
     \label{HB-sum_modified}
 \end{equation}
 
At this point, it is then natural to ask the questions
 \begin{enumerate}
\item How can we generalize Eq.~\ref{HB-sum_modified} to a time varying momentum?
\item Can we understand how do the convergence/ variance reduction properties change when using such time varying momentum? How are these properties affected by normalization? 
 \end{enumerate}

==> sections/old/intoduction_old.tex <==

\section{Introduction}
Our object of study is the classical problem of minimizing finite-sum objective functions of the form
\begin{equation}
    \tag{P}
    x^* = \argmin_{x\in\R^d} f(x):=\frac{1}{n}\sum_{i=1}^nf_i(x).
    \label{P}
\end{equation}


Accelerated gradient methods play a fundamental role in optimizing such objective functions, providing optimal rates of convergence for certain types of function classes such as the ones obeying convex~\cite{nesterov2018lectures}.
The two most popular momentum methods are Heavy-ball (HB)~\cite{polyak1964some} and Nesterov's accelerated gradient (NAG)~\cite{nesterov1983method}.
They are based on the fundamental idea of augmenting gradient-based algorithms with a momentum term that uses \textit{previous gradient directions} in order to accelerate convergence, which yields the following type of iterative updates:
\begin{equation}
\tag{HB}
x_{k+1} = x_{k}-\beta_k (x_k-x_{k-1}) - \eta \nabla f(x_k),
\label{HB}
\end{equation}
where $\beta_k\in[0,1]$\footnote{Gradient Descent \cite{cauchy1847methode} can be seen as a special case of \ref{HB} for $\beta_k = 0$.} is the so-called iteration dependent \textit{momentum parameter} and $\eta$ is a small positive number called \textit{learning rate}.

Although both HB and NAG have received a lot of attention in the literature, the idea of acceleration is still not entirely well understood.
%For instance, the original analysis of Nesterov's accelerated gradient reveals little insight into its inner-working. Notably, some recent papers have used ideas from optimization, geometry and differential equations in order to provide further insights on NAG (see e.g. ~\cite{allen2014linear, bubeck2015geometric, su2014differential}). While these works provide interesting insights for convex settings, our understanding of momentum methods on non-convex function remains very limited.
For example. a series of recent work \cite{su2014differential,wibisono2016variational,yang2018physical} has studied these methods from a physical perspective, which yields a connection to damped linear oscillators. Arguably, the insights provided by these works are mostly descriptive and have so far not been able to help with the design of new accelerated algorithms. Furthermore, the above insights do not translate to stochastic optimization settings, where the stability of momentum methods may actually be reduced due to inexact gradient information~\cite{jain2018accelerating, kidambi2018insufficiency}.

%Moreover, these analyses do not justify the need for a vanishing viscosity parameter $\alpha(t) = 3/t$ in \ref{HB-ODE} in order to achieve acceleration \cite{su2014differential} in the continuous and convex setting.
%A related point of view introduced by \cite{wibisono2016variational}, shows how \ref{HB-ODE} solves a variational problem.
% al: following takes too much space, doesn't seem necessary.
%, linking momentum to the important question
%\begin{center}
%    \textit{"what is the optimal way to optimize?"}
%\end{center}

%Sadly, this theory is weakened by the arbitrariness of the introduced variational problem ---which is defined \textit{ad hoc} to give the desired solution. Moreover, none of the arguments above justifies the need for a vanishing viscosity parameter $\alpha(t) = 3/t$ in \ref{HB-ODE} in order to achieve acceleration \cite{su2014differential} in the continuous and convex setting.


 So far, the only existing proofs of convergence for stochastic non-convex settings~\cite{yang2016unified} typically require more restrictive assumptions such as decreasing learning rates\footnote{See Section~\ref{sec:related_work} for a detailed discussion}. As a consequence, existing rates of convergence (summarized in Table~\ref{tb:summary_existing_rates}) do not yield any improvement over the rate of (stochastic) gradient descent.

This lack of theoretical understanding is rather unsatisfying. Why is it that acceleration able to provide faster rates of convergence for convex functions but fails when used on non-convex functions or in a stochastic setting? This question is especially relevant given that momentum techniques (such as Adam~\cite{kingma2014adam}) are commonly used in machine learning in order to optimize non-convex objective functions that arise when training deep neural networks.

In order to address this issue, we here provide an alternative view on the inner workings of momentum methods which is not physically-inspired but instead builds upon the theoretical work on memory gradient diffusion developed by~\cite{cabot2009long} and \cite{ gadat2014long}. In order to leverage this analogy, we first rewrite \ref{HB} as follows
\begin{tcolorbox}
\begin{equation}
\tag{HB-SUM}
\hspace{-1mm}
x_{k+1} = x_k - \eta \sum_{j=0}^{k-1} \left(\prod_{h=j+1}^k\beta_h\right) \nabla f(x_j)- \eta\nabla f(x_k)
\label{HB-SUM}
\end{equation}
\end{tcolorbox}
where $x_0=x_{-1}$ is assumed. That is, at each iteration $k$ the next step is computed using a \textit{weighted average of past gradients} : $x_{k+1} = x_k + \eta\sum_{j=0}^{k} w(j,k) f(x_k))$. In particular, if $\beta_h$ is constant across all iterations, the memory --- which is controlled by the weights --- vanishes exponentially fast. Such averaging provides a cheap way to 1) adapt to the geometry of ill-conditioned problems (also noted in \cite{sutskever13}) and 2) denoise stochastic gradients if the underlying true gradients are changing slowly. 



% As we detail out in Appendix~\ref{sec:unbiasing}, the latter observation led to the introduction of a bias\footnote{}-correction term in the Adam optimizer.

% While this term only constitutes a slight modification of the original HB algorithm, it is precisely that insight upon which we start the following investigations. Particularly, motivated by the vast empirical success of Adam, we study the effect of the bias correction term on the convergence and variance reduction properties of HB. In this regard, we find that the use of memory is a key ingredient in making momentum methods stable which leads us to the development of an algorithmic framework that can incorporate various types of memory very efficiently. Furthermore, our analysis delivers some potential answers regarding the source of divergence of stochastic momentum methods. In summary, our contributions are the following:


%The idea behind memory diffusion is to augment the dynamics of gradient descent with a memory term which is constructed as a weighted average of the drift term along the past of the trajectory.
%As shown in~\cite{gadat2014long}, the use of memory makes the system more stable. This is of course especially interesting given that HB is known to be loose its superiority to gradient descent in a stochastic setting~\cite{jain2018accelerating, kidambi2018insufficiency}.


% \begin{enumerate}
% \item We generalize the continuous-time limit of HB to a bias-corrected ODE that can incorporate various types of memory (Section \ref{sec:mem_fun_grad_forg}). Furthermore, we extend the memory gradient flow to the stochastic setting (Section \ref{sec:stoc_gradients})
% \item We provide convergence guarantees for the memory ODE and SDE on various types o
% f function classes (Section \ref{sec:analysis_discretization}).
% \item By integrating the memory flows we derive a provably convergent discrete-time algorithm that can
% incorporate a broad range of memory functions (Section \ref{sec:disc}). 
% \item Finally, we run several experiments to support our theory with empirical evidence in both deterministic and stochastic settings (Section \ref{sec:experiments}).
% \end{enumerate}


==> sections/old/name.tex <==
\begin{proof}(of Proposition \ref{prop:CONV_HBF_WQC_QG_app})
Define the following parametric energy

$$\EE_{\gamma,\beta}(X(t),t) := e^{\gamma t}\left(\tilde f(X(t))-\tilde f(x^*) + \frac{1}{2}\|V(t) + \beta (X(t)-x^*)\|^2\right),$$
where $\beta$ and $\gamma$ are positive real numbers. First, we compute an upper bound on the infinitesimal diffusion generator of $\EE$.
\begin{equation*}
    \begin{split}
     \mathcal{A}\EE(X(t),V(t),t) &=\underbrace{\partial_t \EE(X(t),V(t),t)}_{\circled{1}} \underbrace{\langle\partial_{x} \EE(X(t),V(t),t), V\rangle dt}_{\circled{2}}\\
    & \ \ \ \ + \underbrace{\left\langle\partial_{v} \EE(X(t),V(t),t), -\alpha V(t)-\alpha \nabla \tilde f(X(t)) \right\rangle dt}_{\circled{3}}\\
    & \ \ \ \ +  \underbrace{\frac{1}{2}\tr\left(\xi(t)\xi(t)^T\partial^2_{(x,v)}\EE(X(t),V(t),t) \  \right)dt}_{\circled{4}}\\
        & \le \underbrace{\gamma e^{\gamma t}\left[\tilde f(X(t))-\tilde f(x^*) + \frac{1}{2}\|V(t) + \beta (X(t)-x^*)\|^2\right]}_{\circled{1}}\\ 
        & \ \ \ + \underbrace{\frac{d}{2}e^{\gamma t}\tilde\sigma_*^2}_{\circled{2}}  + \underbrace{e^{\gamma t} \langle\nabla \tilde f + \beta V + \beta^2 (X-x^*),V\rangle}_{\circled{3}}\\
        & \ \ \ + \underbrace{e^{\gamma t} \langle V+\beta(X-x^*),-\alpha V -\nabla \tilde f \rangle}_{\circled{4}}\\
    \end{split}
\end{equation*}

where in the inequality we used the definition of $\tilde\sigma_*^2$ and Lemma \ref{lemma:CONV_trace_product}.
Next we multiply both sides by $e^{-\gamma t}$ and proceeding with the calculations we get

\begin{equation*}
    \begin{split}
        e^{-\gamma t}\mathscr{A}\EE & = \gamma \tilde f(X(t))-\tilde f(x^*) + \frac{\gamma}{2}\|V(t) + \beta (X(t)-x^*)\|^2\\ 
        & \ \ \ + \frac{d}{2}\tilde\sigma_*^2 +  \langle\nabla \tilde f + \beta V + \beta^2 (X-x^*),V\rangle\\
        & \ \ \ + \langle V+\beta(X-x^*),-\alpha V -\nabla \tildef \rangle\\
        & = \gamma \tilde f(X(t))-\tilde f(x^*) + \frac{\gamma}{2}\|V\|^2 + \frac{\beta^2\gamma}{2} \|X-x^*\|^2 + \beta\gamma\langle V, X-x^*\rangle\\
        & \ \ \ + \frac{d}{2}\tilde\sigma_*^2 + \langle\nabla \tilde f,V\rangle +  \beta \|V\|^2 + \beta^2 \langle V,X-x^* \rangle\\
        & \ \ \ -\alpha \|V\|^2 -\langle \nabla \tilde f, V\rangle -\alpha \beta \langle V,X-x^*\rangle -\beta\langle \nabla \tilde f, X-x^*\rangle.\\ 
        & \le \left(\gamma + \frac{\beta^2\gamma}{\tilde\mu} - \beta \tau\right) \tilde f(X(t))-\tilde f(x^*) + \frac{d}{2}\tilde\sigma_*^2\\
        & \ \ \  + \left(\frac{\gamma}{2} + \beta -\alpha \right)\|V\|^2 + (\beta\gamma + \beta^2 -\alpha\beta)\langle V, X-x^*\rangle       
    \end{split}
\end{equation*}
where in the inequality we used the $\tilde\mu$-QG assumption and the $\tau$-WQC assumption. Next, since we have no way to bound the term $\langle V,X-x^*\rangle$ in general, we require
$$\gamma\beta + \beta^2 -\alpha\beta = 0.$$
Which holds if and only if $\gamma + \beta = \alpha$. This also implies the coefficient multiplying $\|V\|^2$, that is $\left(\frac{\gamma}{2} + \beta - \alpha\right)$, is negative (because $\gamma$ and $\beta$ are positive).

 
Assume for now that $\left(\gamma + \frac{\beta^2\gamma}{\tilde\mu} - \beta \tau\right)<0$ (we will deal with this at the end of this proof), we get $\mathscr{A}\EE \le \frac{d}{2}\tilde\sigma_*^2e^{\gamma t}.$

Next, using Eq. \ref{eq:dynkin},

$$\E\left[\EE_{\gamma,\beta}(X(t),t)\right] - \EE_{\gamma,\beta}(x_0,0) \le \int_0^t\frac{d}{2}\tilde\sigma_*^2e^{\gamma s} ds.$$


Using the definition of $\EE_{\gamma,\beta}$, we get
\begin{equation}
    e^{\gamma t}\E\left[\tilde f(X(t))-\tilde f(x^*) + \frac{1}{2}\|V(t) + \beta (X(t)-x^*)\|^2\right] \\ \le \tilde f(x_0)-\tilde f(x^*) + \frac{\beta^2}{2}\|(x_0-x^*)\|^2 + \int_0^t\frac{d}{2}\tilde\sigma_*^2e^{\gamma s} ds.
\end{equation}

Hence, discarding the positive term $\frac{1}{2}\|V(t) + \beta (X(t)-x^*)\|^2$ and multiplying both sides by $ e^{-\gamma t}$
\begin{equation}
    \E[\tilde f(X(t))-\tilde f(x^*)]  \le e^{-\gamma t}\left(\tilde f(x_0)-\tilde f(x^*) \frac{\beta^2}{2}\|(x_0-x^*)\|^2\right)\\ + \int_0^t\frac{d}{2}\tilde\sigma_*^2e^{-\gamma (t-s)} ds.
\end{equation}

Which is the statement of the theorem. Now, we just need to choose $\beta$ and $\gamma$ such that $\left(\gamma + \frac{\beta^2\gamma}{\tilde\mu} - \beta \tau\right)<0$ while $\gamma + \beta = \alpha$. Since we have an inequality, we expect that the choice of $\beta$ and $\gamma$ is not unique. However, since $\gamma$ directly influences the rate, we would like it to be as large as possible. This can be formulated with the following linear program with nonlinear constrains.

\begin{equation*}
   (\gamma^*, \beta^*) = \begin{cases}
    \max_{\gamma, \beta} \ \ \ \gamma\\
    \text{s.t} \ \ \ \ \ \ \ \ \ \ \  \gamma = \alpha - \beta\\
    \ \ \ \ \ \ \ \ \ \ \ \ \ \ \  \gamma\le\frac{\tau\beta}{1 + \frac{\beta^2}{\tilde\mu}}\\
    \ \ \ \ \ \ \ \ \ \ \ \ \ \ \  \gamma, \beta > 0
    \end{cases}
\end{equation*}

Using Lemma \ref{lemma:CONV_HBF_WQC_QG}, we shrink the feasible region at the cost of having a suboptimal, yet simpler, solution

\begin{equation*}
   (\gamma^*, \beta^*) = \begin{cases}
    \max_{\gamma, \beta} \ \ \ \gamma\\
    \text{s.t} \ \ \ \ \ \ \ \ \ \ \  \gamma = \alpha - \beta \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \  \ \ (\bigcirc)\\
    \ \ \ \ \ \ \ \ \ \ \ \ \ \ \  \gamma\le \min\left\{\frac{\tau}{2}\beta, \frac{\tau\tilde\mu}{2\beta}\right\} \ \ \ \ \ \ \ (\msquare) \\
    \ \ \ \ \ \ \ \ \ \ \ \ \ \ \  \gamma, \beta > 0
    \end{cases}
\end{equation*}


\begin{figure}
  \centering
    \includegraphics[width=0.6\textwidth]{img/bound_beta_2.pdf}
     \caption{Bounds provided in Lemma \ref{lemma:CONV_HBF_WQC_QG}. Shown is the feasible region for the $\gamma$ maximization problem along with the optimal and approximate solution.}
	\label{fig:bound_beta_2}
\end{figure}

For any fixed $\alpha>0$, the RHS of $(\msquare)$ is positive and the RHS of $(\bigcirc)$ is a line which starts in $(\alpha, 0)$ and eventually exist the set $\{\gamma, \beta) \ : \ \gamma\ge0\}$. Hence, the constrain $(\msquare)$ is binding. The reader can find an helpful representation in Figure \ref{fig:bound_beta_2}. Notice now that we only have one feasible point, hence


\begin{equation*}
   (\gamma^*, \beta^*) = \begin{cases}
    \gamma = \alpha - \beta\\
    \gamma = \min\left\{\frac{\tau}{2}\beta, \frac{\tau\tilde\mu}{2\beta}\right\}\\
    \gamma, \beta > 0
    \end{cases}
\end{equation*}

Next, we ask when $\frac{\tau}{2}\beta = \frac{\tau\tilde\mu}{2\beta}$. This clearly happens at $\beta = \sqrt{\tilde\mu}$. This is the maximum of the continuous curve $\min\left\{\frac{\tau}{2}\beta, \frac{\tau\tilde\mu}{2\beta}\right\}$ with respect to $\beta$. The maximum achievable rate is therefore $\frac{\tau}{2}\sqrt{\tilde\mu}$ and it is reached for $\frac{\tau}{2}\sqrt{\tilde\mu} = \alpha -\sqrt{\tilde\mu} \Rightarrow \alpha = \frac{\tau+2}{2}\sqrt{\tilde\mu}$. Moreover, since $\frac{\tau\tilde\mu}{2\beta}$ and $\frac{\tau}{2}\beta$ only touch in one point, it is clear that

\begin{equation*}
    \gamma^* = 
    \begin{cases}
            \frac{\tau}{2}\beta & \alpha\le\frac{\tau+2}{2}\sqrt{\tilde\mu}\\
            \frac{\tau\tilde\mu}{2\beta} & \alpha\ge\frac{\tau+2}{2}\sqrt{\tilde\mu}
    \end{cases}
\end{equation*}

In any of these two regions, one just has equate the corresponding equation with $\gamma^* = \alpha - \beta^*$, to get




\begin{equation*}
    \gamma^* =\begin{cases}
         \frac{\tau}{\tau +2}\alpha & \text{for }\alpha\le\frac{\tau+2}{2}\sqrt{\tilde\mu} \\
        \frac{1}{2}\left(\alpha-\sqrt{\alpha^2-2\tilde\mu\tau}\right) & \text{for }\alpha\ge\frac{\tau+2}{2}\sqrt{\tilde\mu} \\
    \end{cases}
\end{equation*}

\ 
\end{proof}





==> uai2019_memory (1)/algorithm.tex <==
% ALGORITHM STYLE -- Released 8 April 1996
%    for LaTeX-2e
% Copyright -- 1994 Peter Williams
% E-mail Peter.Williams@dsto.defence.gov.au
\NeedsTeXFormat{LaTeX2e}
\ProvidesPackage{algorithm}
\typeout{Document Style `algorithm' - floating environment}

\RequirePackage{float}
\RequirePackage{ifthen}
\newcommand{\ALG@within}{nothing}
\newboolean{ALG@within}
\setboolean{ALG@within}{false}
\newcommand{\ALG@floatstyle}{ruled}
\newcommand{\ALG@name}{Algorithm}
\newcommand{\listalgorithmname}{List of \ALG@name s}

% Declare Options
% first appearance
\DeclareOption{plain}{
  \renewcommand{\ALG@floatstyle}{plain}
}
\DeclareOption{ruled}{
  \renewcommand{\ALG@floatstyle}{ruled}
}
\DeclareOption{boxed}{
  \renewcommand{\ALG@floatstyle}{boxed}
}
% then numbering convention
\DeclareOption{part}{
  \renewcommand{\ALG@within}{part}
  \setboolean{ALG@within}{true}
}
\DeclareOption{chapter}{
  \renewcommand{\ALG@within}{chapter}
  \setboolean{ALG@within}{true}
}
\DeclareOption{section}{
  \renewcommand{\ALG@within}{section}
  \setboolean{ALG@within}{true}
}
\DeclareOption{subsection}{
  \renewcommand{\ALG@within}{subsection}
  \setboolean{ALG@within}{true}
}
\DeclareOption{subsubsection}{
  \renewcommand{\ALG@within}{subsubsection}
  \setboolean{ALG@within}{true}
}
\DeclareOption{nothing}{
  \renewcommand{\ALG@within}{nothing}
  \setboolean{ALG@within}{true}
}
\DeclareOption*{\edef\ALG@name{\CurrentOption}}

% ALGORITHM
%
\ProcessOptions
\floatstyle{\ALG@floatstyle}
\ifthenelse{\boolean{ALG@within}}{
  \ifthenelse{\equal{\ALG@within}{part}}
     {\newfloat{algorithm}{htbp}{loa}[part]}{}
  \ifthenelse{\equal{\ALG@within}{chapter}}
     {\newfloat{algorithm}{htbp}{loa}[chapter]}{}
  \ifthenelse{\equal{\ALG@within}{section}}
     {\newfloat{algorithm}{htbp}{loa}[section]}{}
  \ifthenelse{\equal{\ALG@within}{subsection}}
     {\newfloat{algorithm}{htbp}{loa}[subsection]}{}
  \ifthenelse{\equal{\ALG@within}{subsubsection}}
     {\newfloat{algorithm}{htbp}{loa}[subsubsection]}{}
  \ifthenelse{\equal{\ALG@within}{nothing}}
     {\newfloat{algorithm}{htbp}{loa}}{}
}{
  \newfloat{algorithm}{htbp}{loa}
}
\floatname{algorithm}{\ALG@name}

\newcommand{\listofalgorithms}{\listof{algorithm}{\listalgorithmname}}



==> uai2019_memory (1)/algorithmic.tex <==
% ALGORITHMIC STYLE -- Released 8 APRIL 1996
%    for LaTeX version 2e
% Copyright -- 1994 Peter Williams
% E-mail PeterWilliams@dsto.defence.gov.au
%
% Modified by Alex Smola (08/2000)
% E-mail Alex.Smola@anu.edu.au
%
\NeedsTeXFormat{LaTeX2e}
\ProvidesPackage{algorithmic}
\typeout{Document Style `algorithmic' - environment}
%
\RequirePackage{ifthen}
\RequirePackage{calc}
\newboolean{ALC@noend}
\setboolean{ALC@noend}{false}
\newcounter{ALC@line}
\newcounter{ALC@rem}
\newlength{\ALC@tlm}
%
\DeclareOption{noend}{\setboolean{ALC@noend}{true}}
%
\ProcessOptions
%
% ALGORITHMIC
\newcommand{\algorithmicrequire}{\textbf{Require:}}
\newcommand{\algorithmicensure}{\textbf{Ensure:}}
\newcommand{\algorithmiccomment}[1]{\{#1\}}
\newcommand{\algorithmicend}{\textbf{end}}
\newcommand{\algorithmicif}{\textbf{if}}
\newcommand{\algorithmicthen}{\textbf{then}}
\newcommand{\algorithmicelse}{\textbf{else}}
\newcommand{\algorithmicelsif}{\algorithmicelse\ \algorithmicif}
\newcommand{\algorithmicendif}{\algorithmicend\ \algorithmicif}
\newcommand{\algorithmicfor}{\textbf{for}}
\newcommand{\algorithmicforall}{\textbf{for all}}
\newcommand{\algorithmicdo}{\textbf{do}}
\newcommand{\algorithmicendfor}{\algorithmicend\ \algorithmicfor}
\newcommand{\algorithmicwhile}{\textbf{while}}
\newcommand{\algorithmicendwhile}{\algorithmicend\ \algorithmicwhile}
\newcommand{\algorithmicloop}{\textbf{loop}}
\newcommand{\algorithmicendloop}{\algorithmicend\ \algorithmicloop}
\newcommand{\algorithmicrepeat}{\textbf{repeat}}
\newcommand{\algorithmicuntil}{\textbf{until}}

%changed by alex smola
\newcommand{\algorithmicinput}{\textbf{input}}
\newcommand{\algorithmicoutput}{\textbf{output}}
\newcommand{\algorithmicset}{\textbf{set}}
\newcommand{\algorithmictrue}{\textbf{true}}
\newcommand{\algorithmicfalse}{\textbf{false}}
\newcommand{\algorithmicand}{\textbf{and\ }}
\newcommand{\algorithmicor}{\textbf{or\ }}
\newcommand{\algorithmicfunction}{\textbf{function}}
\newcommand{\algorithmicendfunction}{\algorithmicend\ \algorithmicfunction}
\newcommand{\algorithmicmain}{\textbf{main}}
\newcommand{\algorithmicendmain}{\algorithmicend\ \algorithmicmain}
%end changed by alex smola

\def\ALC@item[#1]{%
\if@noparitem \@donoparitem
  \else \if@inlabel \indent \par \fi
         \ifhmode \unskip\unskip \par \fi
         \if@newlist \if@nobreak \@nbitem \else
                        \addpenalty\@beginparpenalty
                        \addvspace\@topsep \addvspace{-\parskip}\fi
           \else \addpenalty\@itempenalty \addvspace\itemsep
          \fi
    \global\@inlabeltrue
\fi
\everypar{\global\@minipagefalse\global\@newlistfalse
          \if@inlabel\global\@inlabelfalse \hskip -\parindent \box\@labels
             \penalty\z@ \fi
          \everypar{}}\global\@nobreakfalse
\if@noitemarg \@noitemargfalse \if@nmbrlist \refstepcounter{\@listctr}\fi \fi
\sbox\@tempboxa{\makelabel{#1}}%
\global\setbox\@labels
 \hbox{\unhbox\@labels \hskip \itemindent
       \hskip -\labelwidth \hskip -\ALC@tlm
       \ifdim \wd\@tempboxa >\labelwidth
                \box\@tempboxa
          \else \hbox to\labelwidth {\unhbox\@tempboxa}\fi
       \hskip \ALC@tlm}\ignorespaces}
%
\newenvironment{algorithmic}[1][0]{
\let\@item\ALC@item
  \newcommand{\ALC@lno}{%
\ifthenelse{\equal{\arabic{ALC@rem}}{0}}
{{\footnotesize \arabic{ALC@line}:}}{}%
}
\let\@listii\@listi
\let\@listiii\@listi
\let\@listiv\@listi
\let\@listv\@listi
\let\@listvi\@listi
\let\@listvii\@listi
  \newenvironment{ALC@g}{
    \begin{list}{\ALC@lno}{ \itemsep\z@ \itemindent\z@
    \listparindent\z@ \rightmargin\z@ 
    \topsep\z@ \partopsep\z@ \parskip\z@\parsep\z@
    \leftmargin 1em
    \addtolength{\ALC@tlm}{\leftmargin}
    }
  }
  {\end{list}}
  \newcommand{\ALC@it}{\addtocounter{ALC@line}{1}\addtocounter{ALC@rem}{1}\ifthenelse{\equal{\arabic{ALC@rem}}{#1}}{\setcounter{ALC@rem}{0}}{}\item}
  \newcommand{\ALC@com}[1]{\ifthenelse{\equal{##1}{default}}%
{}{\ \algorithmiccomment{##1}}}
  \newcommand{\REQUIRE}{\item[\algorithmicrequire]}
  \newcommand{\ENSURE}{\item[\algorithmicensure]}
  \newcommand{\STATE}{\ALC@it}
  \newcommand{\COMMENT}[1]{\algorithmiccomment{##1}}
%changes by alex smola
  \newcommand{\INPUT}{\item[\algorithmicinput]}
  \newcommand{\OUTPUT}{\item[\algorithmicoutput]}
  \newcommand{\SET}{\item[\algorithmicset]}
%  \newcommand{\TRUE}{\algorithmictrue}
%  \newcommand{\FALSE}{\algorithmicfalse}
  \newcommand{\AND}{\algorithmicand}
  \newcommand{\OR}{\algorithmicor}
  \newenvironment{ALC@func}{\begin{ALC@g}}{\end{ALC@g}}
  \newenvironment{ALC@main}{\begin{ALC@g}}{\end{ALC@g}}
%end changes by alex smola
  \newenvironment{ALC@if}{\begin{ALC@g}}{\end{ALC@g}}
  \newenvironment{ALC@for}{\begin{ALC@g}}{\end{ALC@g}}
  \newenvironment{ALC@whl}{\begin{ALC@g}}{\end{ALC@g}}
  \newenvironment{ALC@loop}{\begin{ALC@g}}{\end{ALC@g}}
  \newenvironment{ALC@rpt}{\begin{ALC@g}}{\end{ALC@g}}
  \renewcommand{\\}{\@centercr}
  \newcommand{\IF}[2][default]{\ALC@it\algorithmicif\ ##2\ \algorithmicthen%
\ALC@com{##1}\begin{ALC@if}}
  \newcommand{\SHORTIF}[2]{\ALC@it\algorithmicif\ ##1\
    \algorithmicthen\ {##2}}
  \newcommand{\ELSE}[1][default]{\end{ALC@if}\ALC@it\algorithmicelse%
\ALC@com{##1}\begin{ALC@if}}
  \newcommand{\ELSIF}[2][default]%
{\end{ALC@if}\ALC@it\algorithmicelsif\ ##2\ \algorithmicthen%
\ALC@com{##1}\begin{ALC@if}}
  \newcommand{\FOR}[2][default]{\ALC@it\algorithmicfor\ ##2\ \algorithmicdo%
\ALC@com{##1}\begin{ALC@for}}
  \newcommand{\FORALL}[2][default]{\ALC@it\algorithmicforall\ ##2\ %
\algorithmicdo%
\ALC@com{##1}\begin{ALC@for}}
  \newcommand{\SHORTFORALL}[2]{\ALC@it\algorithmicforall\ ##1\ %
    \algorithmicdo\ {##2}}
  \newcommand{\WHILE}[2][default]{\ALC@it\algorithmicwhile\ ##2\ %
\algorithmicdo%
\ALC@com{##1}\begin{ALC@whl}}
  \newcommand{\LOOP}[1][default]{\ALC@it\algorithmicloop%
\ALC@com{##1}\begin{ALC@loop}}
%changed by alex smola
  \newcommand{\FUNCTION}[2][default]{\ALC@it\algorithmicfunction\ ##2\ %
    \ALC@com{##1}\begin{ALC@func}}
  \newcommand{\MAIN}[2][default]{\ALC@it\algorithmicmain\ ##2\ %
    \ALC@com{##1}\begin{ALC@main}}
%end changed by alex smola
  \newcommand{\REPEAT}[1][default]{\ALC@it\algorithmicrepeat%
    \ALC@com{##1}\begin{ALC@rpt}}
    \newcommand{\UNTIL}[1]{\end{ALC@rpt}\ALC@it\algorithmicuntil\ ##1}
  \ifthenelse{\boolean{ALC@noend}}{
    \newcommand{\ENDIF}{\end{ALC@if}}
    \newcommand{\ENDFOR}{\end{ALC@for}}
    \newcommand{\ENDWHILE}{\end{ALC@whl}}
    \newcommand{\ENDLOOP}{\end{ALC@loop}}
    \newcommand{\ENDFUNCTION}{\end{ALC@func}}
    \newcommand{\ENDMAIN}{\end{ALC@main}}
  }{
    \newcommand{\ENDIF}{\end{ALC@if}\ALC@it\algorithmicendif}
    \newcommand{\ENDFOR}{\end{ALC@for}\ALC@it\algorithmicendfor}
    \newcommand{\ENDWHILE}{\end{ALC@whl}\ALC@it\algorithmicendwhile}
    \newcommand{\ENDLOOP}{\end{ALC@loop}\ALC@it\algorithmicendloop}
    \newcommand{\ENDFUNCTION}{\end{ALC@func}\ALC@it\algorithmicendfunction}
    \newcommand{\ENDMAIN}{\end{ALC@main}\ALC@it\algorithmicendmain}
  } 
  \renewcommand{\@toodeep}{}
  \begin{list}{\ALC@lno}{\setcounter{ALC@line}{0}\setcounter{ALC@rem}{0}%
      \itemsep\z@ \itemindent\z@ \listparindent\z@%
      \partopsep\z@ \parskip\z@ \parsep\z@%
      \labelsep 0.5em \topsep 0.2em%
      \ifthenelse{\equal{#1}{0}}
      {\labelwidth 0.5em }
      {\labelwidth  1.2em }
      \leftmargin\labelwidth \addtolength{\leftmargin}{\labelsep}
      \ALC@tlm\labelsep
      }
    }
  {\end{list}}
















==> uai2019_memory (1)/defs.tex <==
% Operators
\usepackage{microtype}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{booktabs}  % used for nice looking tables
\usepackage{color}
\usepackage{graphicx}
\usepackage{float}
\usepackage{mathtools}
\usepackage{mathrsfs}  
\usepackage{tikz}
\usepackage{scalerel}
\usepackage{subcaption}
\usepackage{enumerate}
\usepackage{enumitem}
%\usepackage{hyperref}
\newcommand{\theHalgorithm}{\arabic{algorithm}}
\usepackage{tcolorbox}
\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
\usepackage[utf8]{inputenc}
\usepackage[export]{adjustbox}
\usepackage[T1]{fontenc}


\usepackage[export]{adjustbox}


\makeatletter
\def\BState{\State\hskip-\ALG@thistlm}
\makeatother

\setlist[2]{noitemsep} % sets the itemsep and parsep for all level two lists to 0
\setenumerate{noitemsep} % sets no itemsep for enumerate lists only
\usepackage{cancel}


\newcommand{\cov}[2]{\text{Cov}\left[#1, #2\right]}
\newcommand*\diff{\mathop{}\!\mathrm{d}}
\newcommand{\dw}{\nabla_{\w}}
\newcommand{\fhat}{\hat{f}}
\newcommand{\tf}{\tilde{f}}
\newcommand{\Jhat}{\hat{J}}
\newcommand{\sign}{\text{sign}}
\newcommand{\sqnorm}[1]{\left\|#1\right\|^2} 
\newcommand{\tr}{\text{Tr}}
\newcommand{\vectornorm}[1]{\left\|#1\right\|}
\newcommand{\norm}[1]{{}\left\| #1 \right\|}
\DeclareMathOperator{\var}{Cov}
\DeclareMathOperator*{\argmin}{arg\,min}
\newcommand{\T}{\mathfrak{T}}
\newcommand{\EE}{\mathcal{E}}
\newcommand{\G}{\mathcal{G}}
\newcommand{\OO}{\mathcal{O}}

% Vectors
\newcommand{\av}{{\bf a}}
\newcommand{\eb}{{\bf e}}
\newcommand{\g}{{\bf g}}
\newcommand{\gb}{\bar{g}}
\newcommand{\h}{{\bf h}}
\newcommand{\mutil}{\tilde{\mu}}
\newcommand{\p}{{\bf p}}
\newcommand{\s}{{\bf s}}
\newcommand{\shat}{\hat{s}}
\renewcommand{\u}{{\bf u}}
\newcommand{\vb}{{\bf v}}
\newcommand{\vt}{{\bf v}_t}
\newcommand{\w}{{\bf w}}
\newcommand{\we}{\tilde{\w}}
\newcommand{\wstar}{\w^*}
\newcommand{\wtil}{{\tilde{\bf w}}}
\newcommand{\x}{{\bf x}}
\newcommand{\y}{{\bf y}}
\newcommand{\z}{{\bf z}}
\newcommand{\yhat}{\hat{y}}

\newcommand{\xavg}{{\bf \bar{x}_T}}
\newcommand{\xavgn}{{\bf \bar{x}_n}}
\newcommand{\xavgb}{{\bf \bar{x}_T^{\prime}}}
\newcommand{\xsuffixavg}{{\bf \bar{x}_T^{\alpha}}}
\newcommand{\xstar}{{\bf x^*}}


% Matrices
\def\Am{{\bf A}}
\def\Bm{{\bf B}}
\def\Cm{{\bf C}}
\def\Gm{{\bf G}}
\def\Hm{{\bf H}}
\def\Im{{ I}}
\def\Pm{{\bf P}}
\def\Qm{{\bf Q}}
\def\Rm{{\bf R}}
\def\Zm{{\bf Z}}
\def\Ym{{\bf Y}}
\def\Xm{{\bf X}}


% Sets
\newcommand{\m}{{\mathfrak{m}}}

\newcommand{\A}{{\mathcal A}}
\newcommand{\B}{{\mathcal B}}
\newcommand{\C}{{\mathcal C}}
\newcommand{\D}{{\mathfrak D}}
\newcommand{\E}{{\mathbb E}}
\newcommand{\Efull}{\mathbb{E}}
\newcommand{\F}{{\mathcal F}}
\newcommand{\N}{{\mathbb N}}
\newcommand{\R}{{\mathbb{R}}}
\renewcommand{\S}{{\mathcal S}}
\newcommand{\X}{{\mathcal{X}}}
\newcommand{\Z}{{\mathbf Z}}

% Theorems
\usepackage{mdframed}
\newtheorem*{theorem*}{Theorem}
\newmdtheoremenv{theorem}{Theorem}[section]
\newmdtheoremenv{lemma}[theorem]{Lemma}
\newmdtheoremenv{proposition}[theorem]{Proposition}
\newmdtheoremenv{corollary}[theorem]{Corollary}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{definition}{Definition}[section]
\newtheorem{lemmama}{Lemma}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{example}{Example}[section]

% Comments
\newcommand{\note}[1]{{\textbf{\color{red}#1}}}
\newcommand{\highlight}[1]{\textcolor{red}{#1}}

% Algorithms
\newcommand{\INDSTATE}[1]{\STATE \hspace{2mm} #1}

% Misc
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=2pt] (char) {#1};}}
\def\msquare{\mathord{\scalerel*{\Box}{gX}}}            

\definecolor{colorantonio}{RGB}{0,128,255}

\newcommand{\antonio}[1]{{\color{colorantonio}[Antonio: #1]}}
\newcommand\jonas[1]{{\color{orange}Jonas: ``#1''}}
\newcommand\aurelien[1]{{\color{olive}Aurelien: ``#1''}}
\tcbset{colframe=white}

==> uai2019_memory (1)/sections/experiments.tex <==
\section{LARGE SCALE EXPERIMENTS} \label{sec:experiments}
\vspace{-1mm}
In order to assess the effect of different types of memory in practical settings, we benchmark MemSGD with different memory functions: from instantaneous to exponential, including various types of polynomial forgetting. As a reference point, we also run vanilla \ref{HB} with constant momentum as stated in the introduction. To get a broad overview of the performance of each method, we run experiments on a convex logistic regression loss as well as on non-convex neural networks in both a mini- and full-batch setting. Details regarding algorithms, datasets and architectures can be found in App.~\ref{sec:exp_setting}.
\label{sec:exp}
\begin{figure*}[ht]
\centering 
\begin{adjustbox}{center}
\begin{tabular}{c@{}c@{}c@{}c@{}}
        \small{Covtype Logreg} & \small{MNIST Autoencoder} & \small{FashionMNIST MLP} & \small{CIFAR-10 CNN}
          \\
            \includegraphics[width=0.245\linewidth,valign=c]{exp_jonas/log_full_loss_iteration_covtype_SB}&
            \includegraphics[width=0.245\linewidth,valign=c]{exp_jonas/log_full_loss_iteration_mnist_SB}&
            \includegraphics[width=0.245\linewidth,valign=c]{exp_jonas/log_full_loss_iteration_fashion_mnist_SB}&
            \includegraphics[width=0.245\linewidth,valign=c]{exp_jonas/log_full_loss_iteration_cifar_SB}\\  
            ~
             \includegraphics[width=0.245\linewidth,valign=c]{exp_jonas/log_full_loss_iteration_covtype_LB}&
            \includegraphics[width=0.245\linewidth,valign=c]{exp_jonas/log_full_loss_iteration_mnist_LB}&
            \includegraphics[width=0.245\linewidth,valign=c]{exp_jonas/log_full_loss_iteration_fashion_mnist_LB}&
            \includegraphics[width=0.245\linewidth,valign=c]{exp_jonas/log_full_loss_iteration_cifar_LB}\\  
\end{tabular}
\end{adjustbox}
\vspace{-1mm}
\caption{\footnotesize{Log loss over iterations in mini- (top) and full-batch (bottom) setting. Average and $95\%$ CI of 10 random initializations.}}
\label{fig:results_iterations_main}
\end{figure*}

\vspace{-2mm}
\paragraph{Results and discussion.} Fig.~\ref{fig:results_iterations_main} summarizes our results in terms of training loss. While it becomes evident that no method is best on all problems, we can nevertheless draw some interesting conclusions. 

First, we observe that while long-term memory (especially $p=2$) is faster than SGD in the convex case, it does not provide any empirical gain in the neural network settings. This is not particularly surprising since past gradients may quickly become outdated in non-convex landscapes. Short term memory is at least as good as SGD in all cases except for the CIFAR-10 CNN, which represents the most complex of our loss landscapes in terms of curvature.

Secondly, we find that the best stepsize for \ref{HB} is always strictly smaller than the one for SGD in the non-convex setting. MemSGD, on the other hand, can run on stepsizes as large as SGD which reflects the gradient amplification of \ref{HB} as well as the unbiasedness of MemSGD. Interestingly, however, a closer look at Fig.~\ref{fig:exp_stepnorm} (appendix) reveals that \ref{HB} (with best stepsize) actually takes much smaller steps than SGD for almost all iterations. While this makes sense from the perspective that memory averages past gradients, it is somewhat counter-intuitive given the inertia interpretation of \ref{HB} which should make the method travel further than SGD. Indeed, both \cite{sutskever13} and \cite{goodfellow2016deep} attribute the effectiveness of \ref{HB} to its increased velocity along consistent directions (especially early on in the optimization process). However, our observation, together with the fact that MemSGD with fast forgetting ($p=e$ and $p=100$) is as good as HB, suggests that there is actually more to the success of taking past gradients into account and that this must lie in the altered directions that adapt better to the underlying geometry of the problem.\footnote{Note that we find the exact opposite in the convex case, where \ref{HB} does take bigger steps and converges faster.}

Finally, we draw two conclusions that arise when comparing the mini- and full batch setting. First, the superiority of \ref{HB} and fast forgetting MemSGD over vanilla SGD in the deterministic setting is indeed reduced as soon as stochastic gradients come into play (this is in line with the discussion in Sec. \ref{nesterov_comparison}). Second, we find that stochasticity per se is not needed to optimize the neural networks in the sense that all methods eventually reach very similar methods of suboptimality. That is, not even the full batch methods get stuck in any elevated local minima including the saddle found in the MNIST autoencoder which they nicely escape (given the right stepsize).
\section{MEMORY IN ADAPTIVE METHODS}
\label{padam}
\vspace{-1mm}
While the main focus of this paper is the study of the effect of different types of memory on the \emph{first moment} of the gradients, past gradient information is also commonly used to adapt stepsizes. This is the case for Adagrad and Adam which both make use of the second moment of past gradients to precondition their respective update steps. 

Of course, the use of polynomial memory generalizes directly to the second moment estimates and we thus consider a comprehensive study of the effect of long- versus short-term memory in adaptive preconditioning an exciting direction of future research. In fact, as shown in \cite{reddi2018} the non-convergence issue of Adam can be fixed by making the method forget past gradients less quickly. For that purpose the authors propose an algorithm called AdamNC that essentially differs from Adam by the choice of $\beta_2=1-1/k$, which closely resembles Adagrad with constant memory. Interestingly, the memory framework introduced in this paper allows to interpolate between the two extremes of constant- and exponential memory (i.e. Adagrad and Adam) in a principled way. Indeed, by tuning the additional parameter $p$ --- which specifies the degree of the polynomial memory function --- one can equip Adam with any degree of short- to long-term memory desired. As a proof of concept, Fig.~\ref{fig:padam} shows that Adam equipped with a polynomial memory of the squared gradients (PolyAdam) can in fact be faster than both Adam and Adagrad.


\label{sec:adaptive}
\vspace{-2mm}
\begin{figure}[H]
\centering 
\begin{adjustbox}{center}
\begin{tabular}{c@{}c@{}}
\includegraphics[width=0.49\linewidth,valign=c]{exp_jonas/log_full_loss_iteration_padamwithadagrad}&
\includegraphics[width=0.49\linewidth,valign=c]{exp_jonas/full_train_acc_iteration_padamwithadagrad}\\
\end{tabular}
\end{adjustbox}
\vspace{-2mm}
 \caption{\footnotesize{Cifar-10 CNN: Log loss over iterations (left) and training accuracy (right). Average and $95\%$ confidence interval of 10 runs with random initialization.}}\label{fig:padam}
\end{figure}
\section{CONCLUSION}
\vspace{-1mm}
We undertook an extensive theoretical study of the role of memory in (stochastic) optimization. We provided convergence guarantees for memory systems as well as for novel algorithms based on such systems. This study led us to derive novel insights on momentum methods. We complemented these findings with empirical results, both on simple functions as well as more complex functions based on neural networks. There, long- and short-term memory methods exhibit a different behaviour, which suggests further investigation is needed to better understand the interplay between the geometry of neural networks losses, memory and gradient stochasticity. On a more theoretical side, an interesting direction of future work is the study of the role of memory in state-of-the art momentum methods such as algorithms that include primal averaging, increasing gradient sensitivity or decreasing learning rates (see e.g. \cite{krichene2017acceleration}).


%Existing analysis did not justify the need for a vanishing viscosity parameter $\alpha(t) = 3/t$ in \ref{HB-ODE} in order to achieve acceleration \cite{su2014differential} in the continuous and convex setting.

==> uai2019_memory (1)/sections/introduction.tex <==

\section{INTRODUCTION}
Our object of study is the classical problem of minimizing finite-sum objective functions:
\begin{equation}
    \tag{P}
    x^* = \argmin_{x\in\R^d} f(x):=\frac{1}{n}\sum_{i=1}^nf_i(x).
    \label{P}
\end{equation}

Accelerated gradient methods play a fundamental role in optimizing such losses, providing optimal rates of convergence for certain types of function classes such as the ones being convex~\cite{nesterov2018lectures}.
The two most popular momentum methods are Heavy-ball (\ref{HB})~\cite{polyak1964some} and Nesterov's accelerated gradient (NAG)~\cite{nesterov1983method}.
They are based on the fundamental idea of augmenting gradient-based algorithms with a momentum term that uses \textit{previous gradient directions} in order to accelerate convergence, which yields the following type of iterative updates:
\begin{equation}
\tag{HB}
x_{k+1} = x_{k}+\beta_k (x_k-x_{k-1}) - \eta \nabla f(x_k),
\label{HB}
\end{equation}
with $\beta_k$ an iteration dependent \textit{momentum parameter}\footnote{Gradient Descent~\cite{cauchy1847methode} can be seen as a special case of \ref{HB} for $\beta_k = 0$.} and $\eta$ a positive number called \textit{learning rate} (a.k.a. \textit{stepsize}).

Although both \ref{HB} and NAG have received a lot of attention in the literature, the idea of acceleration is still not entirely well understood.
%For instance, the original analysis of Nesterov's accelerated gradient reveals little insight into its inner-working. Notably, some recent papers have used ideas from optimization, geometry and differential equations in order to provide further insights on NAG (see e.g. ~\cite{allen2014linear, bubeck2015geometric, su2014differential}). While these works provide interesting insights for convex settings, our understanding of momentum methods on non-convex function remains very limited.
For instance, a series of recent works~\cite{su2014differential,wibisono2016variational,yang2018physical} has studied these methods from a physical perspective, which yields a connection to damped linear oscillators. Arguably, the insights provided by these works are mostly descriptive and have so far not been able to help with the design of conceptually new algorithms. Furthermore, the resulting analysis often cannot be easily translated to stochastic optimization settings, where stability of momentum methods may actually be reduced due to inexact gradient information~\cite{jain2018accelerating, kidambi2018insufficiency}.

%Moreover, these analyses do not justify the need for a vanishing viscosity parameter $\alpha(t) = 3/t$ in \ref{HB-ODE} in order to achieve acceleration \cite{su2014differential} in the continuous and convex setting.
%A related point of view introduced by \cite{wibisono2016variational}, shows how \ref{HB-ODE} solves a variational problem.
% al: following takes too much space, doesn't seem necessary.
%, linking momentum to the important question
%\begin{center}
%    \textit{"what is the optimal way to optimize?"}
%\end{center}

%Sadly, this theory is weakened by the arbitrariness of the introduced variational problem ---which is defined \textit{ad hoc} to give the desired solution. Moreover, none of the arguments above justifies the need for a vanishing viscosity parameter $\alpha(t) = 3/t$ in \ref{HB-ODE} in order to achieve acceleration \cite{su2014differential} in the continuous and convex setting.



This lack of theoretical understanding is rather unsatisfying. Why is it that acceleration able to provide faster rates of convergence for convex functions but fails when used on non-convex functions or in a stochastic setting? This question is especially relevant given that momentum techniques (such as Adam~\cite{kingma2014adam}) are commonly used in machine learning in order to optimize non-convex objective functions that arise when training deep neural networks.
%  Given the popularity of momentum methods (such as Adam~\cite{kingma2014adam}) in modern machine learning as well as the fact that accelerated methods do provide faster rates for convex functions in the deterministic case, the lack of a thorough understanding of the behavior of accelerated stochastic gradient methods e.g. on neural network problems is unsatisfying.


In order to address this issue, we here exploit an alternative view on the inner workings of momentum methods which is not physically-inspired but instead builds upon the theoretical work on memory gradient diffusions developed by~\cite{cabot2009long} and~\cite{ gadat2014long}. In order to leverage this analogy, we first rewrite~\ref{HB} as follows:
\begin{tcolorbox}
\vspace{-4mm}
\begin{equation}
\tag{HB-SUM}
\hspace{-1mm}
x_{k+1} = x_k - \eta \sum_{j=0}^{k-1} \left(\prod_{h=j+1}^k\beta_h\right) \nabla f(x_j)- \eta\nabla f(x_k)
\label{HB-SUM}
\end{equation}
\end{tcolorbox}
where $x_0=x_{-1}$ is assumed. That is, at each iteration $k$ the next step is computed using a \textit{weighted average of past gradients} : $x_{k+1} = x_k + \eta\sum_{j=0}^{k} w(j,k) \nabla f(x_k))$. In particular, if $\beta_h$ is constant across all iterations, the memory --- which is controlled by the weights --- vanishes exponentially fast (short-term memory). Such averaging provides a cheap way to 1) adapt to the geometry of ill-conditioned problems (also noted in~\cite{sutskever13}) and 2) denoise stochastic gradients if the underlying true gradients are changing slowly. Similarly, adaptive methods~\cite{duchi2011adaptive,kingma2014adam} use memory of past square gradients to automatically adjust the learning rate during training. For the latter task, it has been shown~\cite{reddi2018} that some form of long-term memory is convenient both for in theory (to ensure convergence) and in practice, since it has been observed that, in a mini-batch setting, \textit{large gradients are not common and might be quite informative}. 

In summary --- most modern stochastic optimization methods can be seen as composition of memory systems. Inspired by this observation and by the undeniable importance of shining some light on the acceleration phenomenon, we make the following contributions.
\vspace{-5mm}
\begin{enumerate}
    \item  Following previous work from \cite{cabot2009long}, we generalize the continuous-time limit of \ref{HB} to an interpretable ODE that can implement various types of gradient forgetting (Sec.~\ref{sec:mem_fun_grad_forg}). Next, we extend this ODE to the stochastic setting (Sec.~\ref{sec:stoc_gradients}). 
    \item By comparing the resulting SDE to the model for Nesterov momentum developed in~\cite{su2014differential}, we provide a novel interpretation of acceleration as gradient amplification and give some potential answers regarding the source of instability of stochastic momentum methods (Sec.~\ref{nesterov_comparison}).
    \item We study the convergence guarantees of our continuous-time memory system and show that, in the convex setting, long-term (polynomial) memory is more stable than classical momentum (Sec.~\ref{sec:analysis_discretization}).
    \item We discretize this memory system and derive an algorithmic framework that can incorporate various types of gradient forgetting efficiently. Crucially, we show the discretization process preserves the convergence guarantees.
    \item We run several experiments to support our theory with empirical evidence in both deterministic and stochastic settings (Sec.~\ref{sec:experiments}).
    \item We propose a modification of Adam which uses long-term memory of gradient second moments to adaptively choose the learning rates (Sec.~\ref{padam}).
\end{enumerate}
\vspace{-3mm}
We provide an overview of our notation in App. \ref{notation}.


% \item 
% \item We provide convergence guarantees for the memory ODE and SDE on various types o
% f function classes (Sec. \ref{sec:analysis_discretization}).
% \item By integrating the memory flows we derive a provably convergent discrete-time algorithm that can
% incorporate a broad range of memory functions (Sec. \ref{sec:disc}). 
% \item Finally, we run several experiments to support our theory with empirical evidence in both deterministic and stochastic settings (Sec. \ref{sec:experiments}).
% \end{enumerate}





% As we detail out in Appendix~\ref{sec:unbiasing}, the latter observation led to the introduction of a bias\footnote{}-correction term in the Adam optimizer.

% While this term only constitutes a slight modification of the original HB algorithm, it is precisely that insight upon which we start the following investigations. Particularly, motivated by the vast empirical success of Adam, we study the effect of the bias correction term on the convergence and variance reduction properties of HB. In this regard, we find that the use of memory is a key ingredient in making momentum methods stable which leads us to the development of an algorithmic framework that can incorporate various types of memory very efficiently. Furthermore, our analysis delivers some potential answers regarding the source of divergence of stochastic momentum methods. In summary, our contributions are the following:


%The idea behind memory diffusion is to augment the dynamics of gradient descent with a memory term which is constructed as a weighted average of the drift term along the past of the trajectory.
%As shown in~\cite{gadat2014long}, the use of memory makes the system more stable. This is of course especially interesting given that HB is known to be loose its superiority to gradient descent in a stochastic setting~\cite{jain2018accelerating, kidambi2018insufficiency}.


% \begin{enumerate}

% \item We provide convergence guarantees for the memory ODE and SDE on various types o
% f function classes (Sec. \ref{sec:analysis_discretization}).
% \item By integrating the memory flows we derive a provably convergent discrete-time algorithm that can
% incorporate a broad range of memory functions (Sec. \ref{sec:disc}). 
% \item Finally, we run several experiments to support our theory with empirical evidence in both deterministic and stochastic settings (Sec. \ref{sec:experiments}).
% \end{enumerate}



==> uai2019_memory (1)/sections/old/OLD_background.tex <==
\section{Memory perspective on HB}
\label{sec:background}

We provide an alternative view on momentum methods which builds on top of the theoretical work on memory gradient diffusion developed by~\cite{cabot2009long, gadat2014long}. First, we rewrite \ref{HB} (initialized with $x_0=x_{-1}$) as
\begin{tcolorbox}
\begin{equation}
\tag{HB-SUM}
\hspace{-1mm}
x_{k+1} = x_k - \eta \sum_{j=0}^{k-1} \left(\prod_{h=j+1}^k\beta_h\right) \nabla f(x_j)- \eta\nabla f(x_k)
\label{HB-SUM}
\end{equation}
\end{tcolorbox}
that is, at iteration $k$ we decide the next step using a weighted average of past gradients: in particular, if $\beta_i$ is constant, the memory vanishes exponentially fast. Such averaging provides a cheap way to 1) adapt to the geometry of ill-conditioned problems (also noted in \cite{sutskever13}) and 2) denoise stochastic gradients if the underlying true gradients are changing slowly. The latter observation led to the introduction of the bias-correction term in ADAM \cite{kingma2014adam}; we remind the reasoning behind it in the next few lines.

In the limit case where true gradients are constant, the averaging procedure in \ref{HB-SUM} is biased: let $i_j\in[N]$ be the data-point selected at iteration $j$ and $\nabla f_{i_j}$ the corresponding stochastic gradient; if we define $\epsilon_j:= \nabla f(x_j)-\nabla f_{i_j}(x_j)$ and pick constant momentum $\beta_j = \beta$, we have
\begin{align*}
    \E\left[\sum_{j=0}^{k} \beta^{k-j} \nabla f_{i_j}(x_j)\right] &= \sum_{j=0}^{k} \beta^{k-j} \E[\nabla f + \epsilon_j]\\
    &= \frac{\beta^{k+1}-1}{\beta -1} \nabla f. 
\end{align*}
Therefore ---to ensure an unbiased update, at least for this simple case--- \cite{kingma2014adam} normalize the sum above  by $\frac{\beta^{k+1}-1}{\beta -1}$, showing significant benefits in the experimental section. Indeed, such normalization retains all the celebrated geometric properties of momentum, while improving statistical accuracy  ---a crucial feature of SGD. In addition, we show in Appendix~\ref{sec:app_background} that such normalization also performs variance reduction.

Therefore, supported by the empirical success of ADAM, it seems reasonable to modify standard Heavy Ball (Eq.~\ref{HB-SUM}) with constant momentum to match the ADAM update:
 \begin{equation}
    x_{k+1} = x_k - \eta \frac{\beta-1}{\beta^{k+1}-1} \sum_{j=0}^{k} \beta^{k-j} \nabla f(x_j).
     \label{HB-sum_modified}
 \end{equation}
 
At this point, it is then natural to ask the questions
 \begin{enumerate}
\item How can we generalize Eq.~\ref{HB-sum_modified} to a time varying momentum?
\item Can we understand how do the convergence/ variance reduction properties change when using such time varying momentum? How are these properties affected by normalization? 
 \end{enumerate}

==> uai2019_memory (1)/sections/old/intoduction_old.tex <==

\section{Introduction}
Our object of study is the classical problem of minimizing finite-sum objective functions of the form
\begin{equation}
    \tag{P}
    x^* = \argmin_{x\in\R^d} f(x):=\frac{1}{n}\sum_{i=1}^nf_i(x).
    \label{P}
\end{equation}


Accelerated gradient methods play a fundamental role in optimizing such objective functions, providing optimal rates of convergence for certain types of function classes such as the ones obeying convex~\cite{nesterov2018lectures}.
The two most popular momentum methods are Heavy-ball (HB)~\cite{polyak1964some} and Nesterov's accelerated gradient (NAG)~\cite{nesterov1983method}.
They are based on the fundamental idea of augmenting gradient-based algorithms with a momentum term that uses \textit{previous gradient directions} in order to accelerate convergence, which yields the following type of iterative updates:
\begin{equation}
\tag{HB}
x_{k+1} = x_{k}-\beta_k (x_k-x_{k-1}) - \eta \nabla f(x_k),
\label{HB}
\end{equation}
where $\beta_k\in[0,1]$\footnote{Gradient Descent \cite{cauchy1847methode} can be seen as a special case of \ref{HB} for $\beta_k = 0$.} is the so-called iteration dependent \textit{momentum parameter} and $\eta$ is a small positive number called \textit{learning rate}.

Although both HB and NAG have received a lot of attention in the literature, the idea of acceleration is still not entirely well understood.
%For instance, the original analysis of Nesterov's accelerated gradient reveals little insight into its inner-working. Notably, some recent papers have used ideas from optimization, geometry and differential equations in order to provide further insights on NAG (see e.g. ~\cite{allen2014linear, bubeck2015geometric, su2014differential}). While these works provide interesting insights for convex settings, our understanding of momentum methods on non-convex function remains very limited.
For example. a series of recent work \cite{su2014differential,wibisono2016variational,yang2018physical} has studied these methods from a physical perspective, which yields a connection to damped linear oscillators. Arguably, the insights provided by these works are mostly descriptive and have so far not been able to help with the design of new accelerated algorithms. Furthermore, the above insights do not translate to stochastic optimization settings, where the stability of momentum methods may actually be reduced due to inexact gradient information~\cite{jain2018accelerating, kidambi2018insufficiency}.

%Moreover, these analyses do not justify the need for a vanishing viscosity parameter $\alpha(t) = 3/t$ in \ref{HB-ODE} in order to achieve acceleration \cite{su2014differential} in the continuous and convex setting.
%A related point of view introduced by \cite{wibisono2016variational}, shows how \ref{HB-ODE} solves a variational problem.
% al: following takes too much space, doesn't seem necessary.
%, linking momentum to the important question
%\begin{center}
%    \textit{"what is the optimal way to optimize?"}
%\end{center}

%Sadly, this theory is weakened by the arbitrariness of the introduced variational problem ---which is defined \textit{ad hoc} to give the desired solution. Moreover, none of the arguments above justifies the need for a vanishing viscosity parameter $\alpha(t) = 3/t$ in \ref{HB-ODE} in order to achieve acceleration \cite{su2014differential} in the continuous and convex setting.


 So far, the only existing proofs of convergence for stochastic non-convex settings~\cite{yang2016unified} typically require more restrictive assumptions such as decreasing learning rates\footnote{See Section~\ref{sec:related_work} for a detailed discussion}. As a consequence, existing rates of convergence (summarized in Table~\ref{tb:summary_existing_rates}) do not yield any improvement over the rate of (stochastic) gradient descent.

This lack of theoretical understanding is rather unsatisfying. Why is it that acceleration able to provide faster rates of convergence for convex functions but fails when used on non-convex functions or in a stochastic setting? This question is especially relevant given that momentum techniques (such as Adam~\cite{kingma2014adam}) are commonly used in machine learning in order to optimize non-convex objective functions that arise when training deep neural networks.

In order to address this issue, we here provide an alternative view on the inner workings of momentum methods which is not physically-inspired but instead builds upon the theoretical work on memory gradient diffusion developed by~\cite{cabot2009long} and \cite{ gadat2014long}. In order to leverage this analogy, we first rewrite \ref{HB} as follows
\begin{tcolorbox}
\begin{equation}
\tag{HB-SUM}
\hspace{-1mm}
x_{k+1} = x_k - \eta \sum_{j=0}^{k-1} \left(\prod_{h=j+1}^k\beta_h\right) \nabla f(x_j)- \eta\nabla f(x_k)
\label{HB-SUM}
\end{equation}
\end{tcolorbox}
where $x_0=x_{-1}$ is assumed. That is, at each iteration $k$ the next step is computed using a \textit{weighted average of past gradients} : $x_{k+1} = x_k + \eta\sum_{j=0}^{k} w(j,k) f(x_k))$. In particular, if $\beta_h$ is constant across all iterations, the memory --- which is controlled by the weights --- vanishes exponentially fast. Such averaging provides a cheap way to 1) adapt to the geometry of ill-conditioned problems (also noted in \cite{sutskever13}) and 2) denoise stochastic gradients if the underlying true gradients are changing slowly. 



% As we detail out in Appendix~\ref{sec:unbiasing}, the latter observation led to the introduction of a bias\footnote{}-correction term in the Adam optimizer.

% While this term only constitutes a slight modification of the original HB algorithm, it is precisely that insight upon which we start the following investigations. Particularly, motivated by the vast empirical success of Adam, we study the effect of the bias correction term on the convergence and variance reduction properties of HB. In this regard, we find that the use of memory is a key ingredient in making momentum methods stable which leads us to the development of an algorithmic framework that can incorporate various types of memory very efficiently. Furthermore, our analysis delivers some potential answers regarding the source of divergence of stochastic momentum methods. In summary, our contributions are the following:


%The idea behind memory diffusion is to augment the dynamics of gradient descent with a memory term which is constructed as a weighted average of the drift term along the past of the trajectory.
%As shown in~\cite{gadat2014long}, the use of memory makes the system more stable. This is of course especially interesting given that HB is known to be loose its superiority to gradient descent in a stochastic setting~\cite{jain2018accelerating, kidambi2018insufficiency}.


% \begin{enumerate}
% \item We generalize the continuous-time limit of HB to a bias-corrected ODE that can incorporate various types of memory (Section \ref{sec:mem_fun_grad_forg}). Furthermore, we extend the memory gradient flow to the stochastic setting (Section \ref{sec:stoc_gradients})
% \item We provide convergence guarantees for the memory ODE and SDE on various types o
% f function classes (Section \ref{sec:analysis_discretization}).
% \item By integrating the memory flows we derive a provably convergent discrete-time algorithm that can
% incorporate a broad range of memory functions (Section \ref{sec:disc}). 
% \item Finally, we run several experiments to support our theory with empirical evidence in both deterministic and stochastic settings (Section \ref{sec:experiments}).
% \end{enumerate}


==> uai2019_memory (1)/sections/old/name.tex <==
\begin{proof}(of Proposition \ref{prop:CONV_HBF_WQC_QG_app})
Define the following parametric energy

$$\EE_{\gamma,\beta}(X(t),t) := e^{\gamma t}\left(\tilde f(X(t))-\tilde f(x^*) + \frac{1}{2}\|V(t) + \beta (X(t)-x^*)\|^2\right),$$
where $\beta$ and $\gamma$ are positive real numbers. First, we compute an upper bound on the infinitesimal diffusion generator of $\EE$.
\begin{equation*}
    \begin{split}
     \mathcal{A}\EE(X(t),V(t),t) &=\underbrace{\partial_t \EE(X(t),V(t),t)}_{\circled{1}} \underbrace{\langle\partial_{x} \EE(X(t),V(t),t), V\rangle dt}_{\circled{2}}\\
    & \ \ \ \ + \underbrace{\left\langle\partial_{v} \EE(X(t),V(t),t), -\alpha V(t)-\alpha \nabla \tilde f(X(t)) \right\rangle dt}_{\circled{3}}\\
    & \ \ \ \ +  \underbrace{\frac{1}{2}\tr\left(\xi(t)\xi(t)^T\partial^2_{(x,v)}\EE(X(t),V(t),t) \  \right)dt}_{\circled{4}}\\
        & \le \underbrace{\gamma e^{\gamma t}\left[\tilde f(X(t))-\tilde f(x^*) + \frac{1}{2}\|V(t) + \beta (X(t)-x^*)\|^2\right]}_{\circled{1}}\\ 
        & \ \ \ + \underbrace{\frac{d}{2}e^{\gamma t}\tilde\sigma_*^2}_{\circled{2}}  + \underbrace{e^{\gamma t} \langle\nabla \tilde f + \beta V + \beta^2 (X-x^*),V\rangle}_{\circled{3}}\\
        & \ \ \ + \underbrace{e^{\gamma t} \langle V+\beta(X-x^*),-\alpha V -\nabla \tilde f \rangle}_{\circled{4}}\\
    \end{split}
\end{equation*}

where in the inequality we used the definition of $\tilde\sigma_*^2$ and Lemma \ref{lemma:CONV_trace_product}.
Next we multiply both sides by $e^{-\gamma t}$ and proceeding with the calculations we get

\begin{equation*}
    \begin{split}
        e^{-\gamma t}\mathscr{A}\EE & = \gamma \tilde f(X(t))-\tilde f(x^*) + \frac{\gamma}{2}\|V(t) + \beta (X(t)-x^*)\|^2\\ 
        & \ \ \ + \frac{d}{2}\tilde\sigma_*^2 +  \langle\nabla \tilde f + \beta V + \beta^2 (X-x^*),V\rangle\\
        & \ \ \ + \langle V+\beta(X-x^*),-\alpha V -\nabla \tildef \rangle\\
        & = \gamma \tilde f(X(t))-\tilde f(x^*) + \frac{\gamma}{2}\|V\|^2 + \frac{\beta^2\gamma}{2} \|X-x^*\|^2 + \beta\gamma\langle V, X-x^*\rangle\\
        & \ \ \ + \frac{d}{2}\tilde\sigma_*^2 + \langle\nabla \tilde f,V\rangle +  \beta \|V\|^2 + \beta^2 \langle V,X-x^* \rangle\\
        & \ \ \ -\alpha \|V\|^2 -\langle \nabla \tilde f, V\rangle -\alpha \beta \langle V,X-x^*\rangle -\beta\langle \nabla \tilde f, X-x^*\rangle.\\ 
        & \le \left(\gamma + \frac{\beta^2\gamma}{\tilde\mu} - \beta \tau\right) \tilde f(X(t))-\tilde f(x^*) + \frac{d}{2}\tilde\sigma_*^2\\
        & \ \ \  + \left(\frac{\gamma}{2} + \beta -\alpha \right)\|V\|^2 + (\beta\gamma + \beta^2 -\alpha\beta)\langle V, X-x^*\rangle       
    \end{split}
\end{equation*}
where in the inequality we used the $\tilde\mu$-QG assumption and the $\tau$-WQC assumption. Next, since we have no way to bound the term $\langle V,X-x^*\rangle$ in general, we require
$$\gamma\beta + \beta^2 -\alpha\beta = 0.$$
Which holds if and only if $\gamma + \beta = \alpha$. This also implies the coefficient multiplying $\|V\|^2$, that is $\left(\frac{\gamma}{2} + \beta - \alpha\right)$, is negative (because $\gamma$ and $\beta$ are positive).

 
Assume for now that $\left(\gamma + \frac{\beta^2\gamma}{\tilde\mu} - \beta \tau\right)<0$ (we will deal with this at the end of this proof), we get $\mathscr{A}\EE \le \frac{d}{2}\tilde\sigma_*^2e^{\gamma t}.$

Next, using Eq. \ref{eq:dynkin},

$$\E\left[\EE_{\gamma,\beta}(X(t),t)\right] - \EE_{\gamma,\beta}(x_0,0) \le \int_0^t\frac{d}{2}\tilde\sigma_*^2e^{\gamma s} ds.$$


Using the definition of $\EE_{\gamma,\beta}$, we get
\begin{equation}
    e^{\gamma t}\E\left[\tilde f(X(t))-\tilde f(x^*) + \frac{1}{2}\|V(t) + \beta (X(t)-x^*)\|^2\right] \\ \le \tilde f(x_0)-\tilde f(x^*) + \frac{\beta^2}{2}\|(x_0-x^*)\|^2 + \int_0^t\frac{d}{2}\tilde\sigma_*^2e^{\gamma s} ds.
\end{equation}

Hence, discarding the positive term $\frac{1}{2}\|V(t) + \beta (X(t)-x^*)\|^2$ and multiplying both sides by $ e^{-\gamma t}$
\begin{equation}
    \E[\tilde f(X(t))-\tilde f(x^*)]  \le e^{-\gamma t}\left(\tilde f(x_0)-\tilde f(x^*) \frac{\beta^2}{2}\|(x_0-x^*)\|^2\right)\\ + \int_0^t\frac{d}{2}\tilde\sigma_*^2e^{-\gamma (t-s)} ds.
\end{equation}

Which is the statement of the theorem. Now, we just need to choose $\beta$ and $\gamma$ such that $\left(\gamma + \frac{\beta^2\gamma}{\tilde\mu} - \beta \tau\right)<0$ while $\gamma + \beta = \alpha$. Since we have an inequality, we expect that the choice of $\beta$ and $\gamma$ is not unique. However, since $\gamma$ directly influences the rate, we would like it to be as large as possible. This can be formulated with the following linear program with nonlinear constrains.

\begin{equation*}
   (\gamma^*, \beta^*) = \begin{cases}
    \max_{\gamma, \beta} \ \ \ \gamma\\
    \text{s.t} \ \ \ \ \ \ \ \ \ \ \  \gamma = \alpha - \beta\\
    \ \ \ \ \ \ \ \ \ \ \ \ \ \ \  \gamma\le\frac{\tau\beta}{1 + \frac{\beta^2}{\tilde\mu}}\\
    \ \ \ \ \ \ \ \ \ \ \ \ \ \ \  \gamma, \beta > 0
    \end{cases}
\end{equation*}

Using Lemma \ref{lemma:CONV_HBF_WQC_QG}, we shrink the feasible region at the cost of having a suboptimal, yet simpler, solution

\begin{equation*}
   (\gamma^*, \beta^*) = \begin{cases}
    \max_{\gamma, \beta} \ \ \ \gamma\\
    \text{s.t} \ \ \ \ \ \ \ \ \ \ \  \gamma = \alpha - \beta \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \  \ \ (\bigcirc)\\
    \ \ \ \ \ \ \ \ \ \ \ \ \ \ \  \gamma\le \min\left\{\frac{\tau}{2}\beta, \frac{\tau\tilde\mu}{2\beta}\right\} \ \ \ \ \ \ \ (\msquare) \\
    \ \ \ \ \ \ \ \ \ \ \ \ \ \ \  \gamma, \beta > 0
    \end{cases}
\end{equation*}


\begin{figure}
  \centering
    \includegraphics[width=0.6\textwidth]{img/bound_beta_2.pdf}
     \caption{Bounds provided in Lemma \ref{lemma:CONV_HBF_WQC_QG}. Shown is the feasible region for the $\gamma$ maximization problem along with the optimal and approximate solution.}
	\label{fig:bound_beta_2}
\end{figure}

For any fixed $\alpha>0$, the RHS of $(\msquare)$ is positive and the RHS of $(\bigcirc)$ is a line which starts in $(\alpha, 0)$ and eventually exist the set $\{\gamma, \beta) \ : \ \gamma\ge0\}$. Hence, the constrain $(\msquare)$ is binding. The reader can find an helpful representation in Figure \ref{fig:bound_beta_2}. Notice now that we only have one feasible point, hence


\begin{equation*}
   (\gamma^*, \beta^*) = \begin{cases}
    \gamma = \alpha - \beta\\
    \gamma = \min\left\{\frac{\tau}{2}\beta, \frac{\tau\tilde\mu}{2\beta}\right\}\\
    \gamma, \beta > 0
    \end{cases}
\end{equation*}

Next, we ask when $\frac{\tau}{2}\beta = \frac{\tau\tilde\mu}{2\beta}$. This clearly happens at $\beta = \sqrt{\tilde\mu}$. This is the maximum of the continuous curve $\min\left\{\frac{\tau}{2}\beta, \frac{\tau\tilde\mu}{2\beta}\right\}$ with respect to $\beta$. The maximum achievable rate is therefore $\frac{\tau}{2}\sqrt{\tilde\mu}$ and it is reached for $\frac{\tau}{2}\sqrt{\tilde\mu} = \alpha -\sqrt{\tilde\mu} \Rightarrow \alpha = \frac{\tau+2}{2}\sqrt{\tilde\mu}$. Moreover, since $\frac{\tau\tilde\mu}{2\beta}$ and $\frac{\tau}{2}\beta$ only touch in one point, it is clear that

\begin{equation*}
    \gamma^* = 
    \begin{cases}
            \frac{\tau}{2}\beta & \alpha\le\frac{\tau+2}{2}\sqrt{\tilde\mu}\\
            \frac{\tau\tilde\mu}{2\beta} & \alpha\ge\frac{\tau+2}{2}\sqrt{\tilde\mu}
    \end{cases}
\end{equation*}

In any of these two regions, one just has equate the corresponding equation with $\gamma^* = \alpha - \beta^*$, to get




\begin{equation*}
    \gamma^* =\begin{cases}
         \frac{\tau}{\tau +2}\alpha & \text{for }\alpha\le\frac{\tau+2}{2}\sqrt{\tilde\mu} \\
        \frac{1}{2}\left(\alpha-\sqrt{\alpha^2-2\tilde\mu\tau}\right) & \text{for }\alpha\ge\frac{\tau+2}{2}\sqrt{\tilde\mu} \\
    \end{cases}
\end{equation*}

\ 
\end{proof}





==> uai2019_memory (1)/sections/related_work.tex <==

\section{RELATED WORK}
\label{sec:related_work}
\vspace{-1mm}

\begin{scriptsize}
\begin{table*}
\centering
\begin{tabular}{| l | l | c | c |}
  \hline
   \textbf{Function}& \textbf{Gradient} &  \textbf{Rate} &  \textbf{Reference} \\
 \hline
$\mu$-strongly-convex, $L$-smooth & Deterministic & $f(x_k) -f(x^*) \le \mathcal{O}(q^k)$ & \cite{polyak1964some} \\
Convex, $L$-smooth & Deterministic & $f(\bar{x}_k) -f(x^*) \le \mathcal{O}(1/k)$ & \cite{ghadimi2015global} \\
Convex & Stochastic & $\E\left(f(\bar{x}_k) -f(x^*)\right)\le \mathcal{O}(1/\sqrt{k})$ & \cite{yang2016unified} (*) \\
Non-convex, $L$-smooth & Stochastic & $\min_{i\le k}\E \left[||\nabla f(x_i)||^2\right]\le \mathcal{O} (1/\sqrt{k})$ & \cite{yang2016unified} (*) \\
\hline
\end{tabular}
\caption{\footnotesize{Existing convergence rate for Heavy-ball for general functions (special cases for quadratic functions are mentioned in the main text). The term $\bar{x}_k$ denotes the Cesaro average of the iterates. The constant $q$ is defined as $q = \frac{\sqrt{L}-\sqrt{\mu}}{\sqrt{L}+\sqrt{\mu}}$. (*) The results of~\cite{yang2016unified} also require bounded noise and bounded gradients as well as a step size decreasing as $1/\sqrt{k}$.}}
\label{tb:summary_existing_rates}
\end{table*}
\end{scriptsize}
\paragraph{Momentum in deterministic settings.}
The first accelerated proof of convergence for the deterministic setting dates back to~\cite{polyak1964some} who proved a local linear rate of convergence for Heavy-ball (with constant momentum) for twice continuously differentiable, $\mu$-strongly convex and $L$-smooth functions (with a constant which is faster than gradient descent). \cite{ghadimi2015global} derived a proof of convergence of the same method for convex functions with Lipschitz-continuous gradients, for which the Cesàro average of the iterates converges in function value like $\mathcal{O}(1/k)$ (for small enough $\eta$ and $\beta$).

A similar method, Nesterov's Accelerated Gradient (NAG), was introduced by~\cite{nesterov1983method}. It achieves the optimal $\mathcal{O}(1/k^2)$ rate of convergence for convex functions and, with small modifications, an accelerated (with respect to gradient desacent) linear convergence rate for smooth and strongly-convex functions.

\vspace{-2mm}
\paragraph{Momentum in stochastic settings.}
Prior work has shown that the simple momentum methods discussed above lack stability in stochastic settings, where the evaluation of the gradients is affected by noise~(see motivation in \cite{allen2017katyusha} for the Katyusha method). In particular, for quadratic costs, ~\cite{polyak1987introduction} showed that stochastic Heavy-ball does not achieve any accelerated rate but instead matches the
rate of SGD. More general results are proved in \cite{yang2016unified} for these methods, both for convex and for smooth functions, requiring a decreasing learning rate, bounded noise and bounded subgradients (see Tb.\ref{tb:summary_existing_rates}). For strongly-convex functions,~\cite{yuan2016influence} also studied the mean-square error stability and showed that convergence requires small (constant) learning rates. Furthermore, the rate is shown to be equivalent to SGD and therefore the theoretical  benefits of acceleration in the deterministic setting do not seem to carry over to the stochastic setting.

\vspace{-2mm}
\paragraph{Continuous-time perspective.} The continuous time ODE model of NAG for convex functions presented in~\cite{su2014differential} led to the developments of several variants of Nesterov-inspired accelerated methods in the deterministic setting (e.g.~\cite{krichene2015accelerated} and~\cite{wilson2016lyapunov}). In this line of research, interesting insights often come from a numerical analysis and discretization viewpoint~\cite{zhang2018direct,betancourt2018symplectic}. Similarly, in stochastic settings, guided by SDE models derived from Nesterov's ODE in \cite{su2014differential} and by the variational perspective in~\cite{wibisono2016variational}, ~\cite{xu2018accelerated} and~\cite{xu2018continuous} proposed an interpretable alternative to AC-SA (an accelerated stochastic approximation algorithm introduced in ~\cite{lan2012optimal} and \cite{ghadimi2012optimal}). This is a sophisticated momentum method that in expectation achieves a $\mathcal{O}(L/k^2 + \varsigma_*^2 d/(\mu k))$  rate\footnote{$\varsigma_*^2$ bounds the stochastic gradient variance in each direction.} for $\mu$-strongly convex and $L$-smooth functions and $\mathcal{O}(L/k^2 + \varsigma_*^2 d/\sqrt{k})$ for convex $L$-smooth functions. These rates are nearly optimal, since in the deterministic limit $\varsigma_*\to 0$ they still capture acceleration.

Unlike~\cite{xu2018accelerated,xu2018continuous}, we focus on how the memory of past gradients relates to the \textit{classical} and most widely used momentum methods (\ref{HB}, NAG) and, with the help of the SDE models, show that the resulting insights can be used to design building blocks for new optimization methods. 

%Finally, there exists some results for non-convex functions such as a proof of convergence to a stationary point by~\cite{zavriev1993heavy} and a convergence rate for functions satisfying the so-called Kurdyka-{\L}ojasiewicz (KL) property in~\cite{ochs2014ipiano}. Some results also exist in non-convex stochastic settings such as almost sure convergence in the case of non-convex coercive functions in~\cite{gadat2018stochastic} and a convergence rate for smooth functions in~\cite{yang2016unified} (see Table~\ref{tb:summary_existing_rates}).
%\aurelien{TBD, don't remember which methods use an increasing momentum?} \antonio{NAG for convex, see the second page in \cite{su2014differential}. Also, in \cite{zou2018sufficient} suggest an increasing momentum parameter $\beta_2$ in ADAM (plan to do experiments on this, which they dont do). Also there is this paper https://openreview.net/pdf?id=OM0jvwB8jIp57ZJjtNEZ which basically leaves all as hyperparameter.}

% \paragraph{Results on Quadratic Functions}

% To the best of our knowledge, there is still no global convergence analysis that guarantees an accelerated rate for convex and smooth functions (in the discrete-time setting) or an accelerated linear rate for strongly-convex and smooth functions in the stochastic setting. The only exceptions are~\cite{lessard2016analysis, flammarion2015averaging} for the special case of quadratic functions. Similar results have been obtained by~\cite{loizou2017momentum} on the same type of functions but in a stochastic setting.




% \paragraph{Discretization}
% The problem of discretizing ODEs and SDEs is well-studied and can for instance be solved using Runge-Kutta methods which include the well-known Euler method. An open problem is to discretize a continuous process while preserving the rate of convergence. There are cases where the rate is preserved including the work of~\cite{zhang2018direct} who showed that Runge-Kutta integration generates a discrete-time accelerated method for smooth and convex functions. However, the resulting discrete-time method does not correspond to neither HB nor NAG. ~\cite{betancourt2018symplectic} used symplectic integrators which we will further discuss later on.




==> uai2019_memory (1)/sections/theory.tex <==
\vspace{-1mm}
\section{MEMORY GRADIENT SDE}
\label{sec:MGSDE}
\vspace{-2mm}
In his 1964 paper, Polyak motivated \ref{HB} as the discrete time analogue of a second order ODE:
\begin{tcolorbox}
\vspace{-2mm}
\begin{equation}
    \tag{HB-ODE}
    \ddot X(t) + a(t) \dot X(t) + \nabla f(X(t)) = 0, \ \ 
    \label{HB-ODE}
\end{equation}
\end{tcolorbox}
which can be written in phase-space as
\begin{tcolorbox}
\vspace{-5mm}
\begin{equation}
    \tag{HB-ODE-PS}
    \begin{cases}
    \dot V(t) = -a(t) V(t) -\nabla f(X(t))\\
    \dot X(t) = V(t)
    \end{cases}.
    \label{HB-ODE_PS}
\end{equation}
\vspace{-5mm}
\end{tcolorbox}

This connection can be made precise: in App.~\ref{discretization_HB_proof} we show that \ref{HB} is indeed the result of semi-implicit Euler integration\footnote{~\cite{hairer2006geometric} for an introduction.} on \ref{HB-ODE_PS}.

\subsection{MEMORY AND GRADIENT FORGETTING}
\label{sec:mem_fun_grad_forg}
If the viscosity parameter $\alpha = a(t)$ is time-independent, \ref{HB-ODE}, with initial condition $\dot X(0) = 0$ and $X(0) = x_0$, can be  cast into an integro-differential equation\footnote{By computing $\ddot X$ from \ref{HB-ODE-INT-C} using the fundamental theorem of calculus and plugging in $\dot X(0) = 0$.}:
\begin{tcolorbox}
\vspace{-2mm}
\begin{equation}
    \tag{HB-ODE-INT-C}
    \dot X(t) = -\int_0^t e^{-\alpha \cdot (t-s)} \nabla f(X(s)) ds.
    \label{HB-ODE-INT-C}
\end{equation}
\end{tcolorbox}
\vspace{-1mm}
\paragraph{Bias correction.}
Notice that the instantaneous update direction of \ref{HB-ODE-INT-C} is a weighted average of the past gradients, namely $\int_0^t w(s,t) \nabla f(X(s)) ds$ with $w(s,t) := e^{\alpha(t-s)}$. However, the weights do not integrate to one. Indeed, for all $t$, we have $\int_0^t w(s,t) ds = (1-e^{-\alpha t})/\alpha$, which goes to $1/\alpha$ as $t\to\infty$. As a result, in the constant gradient setting, the previous sum is a \textit{biased estimator} of the actual gradient. This fact suggests a simple modification of \ref{HB-ODE-INT-C}, for $t>0$:
\begin{equation}
   \dot X(t) = -\frac{\alpha}{1-e^{-\alpha t}}\int_0^t e^{-\alpha\cdot(t-s)} \nabla f(X(s)) ds.\label{normalization_step} 
\end{equation}
which we write as $\dot X = -\frac{\alpha}{e^{\alpha t}-1}\int_0^t e^{\alpha s} \nabla f(X(s)) ds$. We note that this normalization step follows exactly the same motivation as bias correction in Adam; we provide an overview of this method in App.~\ref{sec:unbiasing}. If we define $\mathfrak{m}(t) := e^{\alpha t}-1$, the previous formula takes the form:
\begin{tcolorbox}
\vspace{-2mm}
\begin{equation}
\tag{MG-ODE-INT}
    \dot X(t) = -\int_0^t \frac{\dot\m(s)}{\mathfrak{m}(t)} \nabla f(X(s)) ds.
    \label{MG-ODE-INT}
\end{equation}
\end{tcolorbox}
This memory-gradient integro-differential equation (\ref{MG-ODE-INT}) provides a generalization of \ref{HB-ODE-INT-C}, with bias correction. The following crucial lemma is consequence of the fundamental theorem of calculus.
\begin{lemmama}
    For any $\mathfrak{m}\in\C^1(\R,\R)$ s.t. $\mathfrak{m}(0) = 0$, \ref{MG-ODE-INT} is normalized : $\int_0^t \frac{\dot\m(s)}{\m(t)}ds =1$, for all $t > 0$.
    \label{lemma:unbiased}
\end{lemmama}
\vspace{-2em}
\begin{proof}
Since $\mathfrak{m}(0)=0$, $\int_0^t\dot \m(s)ds = \mathfrak{m}(t)$.
\end{proof}
\vspace{-1mm}
Based on Lemma~\ref{lemma:unbiased}, we will always set $\m(0) = 0$. What other properties shall a general $\m(\cdot)$ have? Requiring $\dot \m(s) \neq 0$ for all $s\ge0$ ensures that there does not exist a time instant where the gradient is systematically discarded. Hence, since $\m(0)=0$, $\m(\cdot)$ is either monotonically decreasing and negative or monotonically increasing and positive. In the latter case, without loss of generality, we can flip its sign. This motivates the following definition.
\vspace{-1 mm}
\paragraph{Definition.}
$\m\in\mathcal{C}^1(\R_+,\R)$ is a \textbf{memory function} if it is non-negative, strictly increasing and s.t. $\m(0)=0$.

For example, $e^{\alpha t}-1$, from which we started our discussion, is a valid memory function. Crucially, we note that $\dot \m(\cdot)$ plays the important role of controlling the speed at which we \textit{forget} previously observed gradients. For instance, let $\m(t) = t^3$; since $\dot\m(s) = 3s^2$, the system forgets past gradients \textit{quadratically fast}. In contrast, $\m(t) = e^{\alpha t}-1$ leads to \textit{exponential forgetting}. Some important memory functions are listed in Tb.~\ref{tb:memories}, and their respective influence on past gradients is depicted in Fig.~\ref{fig:memory_types}. We point out that, in the limit $\alpha\to\infty$, the weights $w(s,t) = \frac{\dot\m(s)}{\m(t)}$ associated with exponential forgetting converge to a Dirac distribution $\delta(t-s)$. Hence, we recover the Gradient Descent ODE~\cite{mertikopoulos2018convergence}: $\dot X(t) = -\nabla f(X(t))$. For the sake of comparability, we will refer to this as \textit{instantaneous forgetting}.

Finally, notice that \ref{MG-ODE-INT} can be written as a second order ODE. Too see this, we just need to compute the second derivative. For $t>0$ we have that
$$\ddot X(t) = \frac{\dot\m(t)}{\m(t)^2} \int_0^t\dot \m(s) \nabla f(X(s)) ds - \frac{\dot\m(t)}{\m(t)}\nabla f(X(t)).$$
Plugging in the definition of $\dot X$ from the integro-differential equation, we get the memory-gradient ODE:
\begin{tcolorbox}
\vspace{-5mm}
\begin{equation}
    \tag{MG-ODE}
    \ddot X(t) + \frac{\dot\m(t)}{\m(t)}\dot X(t) + \frac{\dot\m(t)}{\m(t)}\nabla f(X(t)) = 0.
    \label{MG-ODE}
\end{equation}
\vspace{-5mm}
\end{tcolorbox}


\begin{figure}
    \centering
    \includegraphics[width=0.70\linewidth]{img/memory}
    \caption{\footnotesize{Illustration of the influence of past gradients on $\dot X(6)$ (i.e. the right hand side of equation \ref{MG-ODE-INT} with $t=5$). The corresponding memory function can be found in Tb. \ref{tb:memories}. The influence is computed as $\dot\m(s)/\m(6)$. By Lemma \ref{lemma:unbiased}, the area under all curves is 1.}}
    \label{fig:memory_types}
\end{figure}
\begin{table}[ht]
\begin{center}
\begin{tabular}{l|l|l}
\small{\textbf{Forgetting}}  &\small{\textbf{Memory}   $\boldsymbol{\m}$} & \small{\textbf{ODE Coeff. } $\boldsymbol{\dot\m/\m}$} \\
\hline
Decaying    &$\log(1+t)$ & $1/(t\log(t+1))$ \\
Constant    &$t$ & $1/t$ \\
Square-root    &$t^{1.5}$ & $1.5/t$ \\
Linear      &$t^2$ & $2/t$ \\
Quadratic   &$t^3$ & $3/t$ \\
Exponential   &$e^{\alpha t}-1$ & $\alpha e^{\alpha t}/\left(e^{\alpha t}-1\right)$ \\
Super-exp   &$e^{t^\alpha}-1$ & $\alpha t^{\alpha-1} e^{t^\alpha}/\left(e^{t^\alpha}-1\right)$ \\
Instantaneous  &$-$ & $-$ \\
\hline
\end{tabular}
\end{center}
\caption{\footnotesize{Some important examples of memory functions.}}
\label{tb:memories}
\end{table}

Equivalently, we can transform this second order ODE into a system of two first order ODEs by introducing the variable $V(t):=\dot X(t)$ and noting that $\dot V(t) = -\frac{\dot\m(t)}{\m(t)} V(t) -\frac{\dot\m(t)}{\m(t)}\nabla f(X(t))$. This is called the \textit{phase-space representation} of~\ref{MG-ODE}, which we use in Sec.~\ref{sec:stoc_gradients} to provide the extension to the stochastic setting. Also, for the sake of comparison with recent literature~(e.g.~\cite{wibisono2016variational}), we provide a variational interpretation of~\ref{MG-ODE} in App.~\ref{lagrangian}.
\vspace{-2mm}
\paragraph{Existence and uniqueness.}
Readers familiar with ODE theory probably realized that, since by definition $\m(0) = 0$, the question of existence and uniqueness of the solution to~\ref{MG-ODE} is not trivial. This is why we stressed its validity for $t>0$ multiple times during the derivation. Indeed, it turns out that such a solution may not exist globally on $[0,\infty)$ (see App.~\ref{app:counterexample}).  Nevertheless, if we allow to start integration from \textit{any} $\epsilon>0$ and assume $f(\cdot)$ to be $L$-smooth, standard ODE theory~\cite{khalil2002nonlinear} ensures that the sought solution exists and is unique on $[\epsilon,\infty)$. Since $\epsilon$ can be made as small as we like (in our simulations in App.~\ref{app:ODEs_quadratic} we use $\epsilon = 10^{-16}$) this apparent issue can be regarded an artifact of the model. Also, we point out that the integral formulation~\ref{MG-ODE-INT} is well defined for every $t>0$. Therefore, in the theoretical part of this work, we act as if integration starts at $0$ but we highlight in the appendix that choosing the initial condition $\epsilon>0$ induces only a negligible difference (see Remarks~\ref{rmk1_exi} and~\ref{rmk2_exi}).


\subsection{INTRODUCING STOCHASTIC GRADIENTS}
\label{sec:stoc_gradients}
In this section we introduce stochasticity in the~\ref{MG-ODE} model. As already mentioned in the introduction, at each step $k$, iterative stochastic optimization methods have access to an estimate $\G(x_k)$ of $\nabla f(x_k)$: the so called \textit{stochastic gradient}. This information is used and possibly combined with previous gradient estimates $\G(x_0),\dots, \G(x_{k-1})$, to compute a new approximation $x_{k+1}$ to the solution $x^*$. There are many ways to design $\G(k)$: the simplest~\cite{robbins1951stochastic} is to take $\mathcal{G}_{\text{MB}}(x_k) := \nabla f_{i_k}(x_k)$,
where $i_k \in \{1,\dots,n\}$ is a uniformly sampled datapoint. This gradient estimator is trivially unbiased (conditioned on past iterates) and we denote its covariance matrix at point $x$ by $\Sigma(x) = \frac{1}{n}\sum_{i=1}^n (\nabla f_i(x)-\nabla f(x))(\nabla f_i(x)-\nabla f(x))^T$.

Following~\cite{krichene2017acceleration} we model such stochasticity adding a volatility term in \ref{MG-ODE}.

\begin{tcolorbox}
\vspace{-5mm}
\small{
\begin{equation}
    \tag{MG-SDE}
    \begin{cases}
    dX(t) = V(t) dt\\ 
    dV(t) = -\frac{\dot \m(t)}{\m (t)}V(t)dt\\
    \ \ \ \ \ \ \ \ \ \ \ \ \ \ \  -\frac{\dot \m(t)}{\m (t)}\left[\nabla f(X(t))dt +\sigma(X(t)) dB(t)\right]
    \end{cases}
    \label{MG-SDE}
\end{equation}
}
\vspace{-5mm}
\end{tcolorbox}
where $\sigma(X(t))\in\R^{d\times d}$ and $\{B(t)\}_{t\ge0}$ is a standard Brownian Motion. Notice that this system of equations reduces to the phase-space representation of \ref{MG-ODE} if $\sigma(X(t))$ is the null matrix. The connection from $\sigma(x)$ to the gradient estimator covariance matrix $\Sigma(x)$ can be made precise: \cite{li2017stochastic} motivate the choice  $\sigma(x) = \sqrt{h\Sigma(x)}$, where $\sqrt{\cdot}$ denotes the principal square root and $h$ is the discretization stepsize. 

The proof of existence and uniqueness to the solution of this SDE\footnote{See e.g. Thm. 5.2.1 in \cite{oksendal2003stochastic}, which gives sufficient conditions for (strong) existence and uniqueness.} relies on the same arguments made for \ref{MG-ODE} in Sec. \ref{sec:mem_fun_grad_forg}, with one additional crucial difference: \cite{orvieto2018continuous} showed that $f(\cdot)$ needs to additionally be three times continuously differentiable with bounded third derivative (i.e. $f\in\C^3_b(\R^d,\R)$), in order for $\sigma(\cdot)$ to be Lipschitz continuous. Hence, we will assume this regularity and refer the reader to~\cite{orvieto2018continuous} for further details.


% The distribution of the stochastic process $\{(X(t),V(t))\}_{t\ge0}$ has already received a lot of attention from the stochastic analysis community (see e.g. \cite{cabot2009long,gadat2014long}). In this work, we instead focus on the analysis of population quantities  (Sec. \ref{sec:conv_SDE}), on stability issues and on comparison with momentum methods in optimization (Sec. \ref{nesterov_comparison}), on provably convergent discretization (Sec. \ref{sec:discretization}), on the connection to adaptive methods (\ref{sec:adaptive}) and  on experimental evaluation in large scale learning (Sec.  \ref{sec:exp}).


\subsection{THE CONNECTION TO NESTEROV'S SDE}
\label{nesterov_comparison}
\cite{su2014differential} showed that the continuous-time limit of NAG for convex functions is \ref{HB-ODE} with time-dependent viscosity $3/t$: $\ddot X(t) +\frac{3}{t}\dot X(t) + \nabla f(X(t))=0$, which we refer to as \textit{Nesterov's ODE}. Using Bessel functions, the authors were able to provide a new insightful description and analysis of this mysterious algorithm. In particular, they motivated how the vanishing viscosity is essential for acceleration\footnote{Acceleration is not achieved for a viscosity of e.g. $2/t$.}. Indeed, the solution to the equation above is s.t. $f(X(t))-f(x^*) \le \OO(1/t^2)$; in contrast to the solution to the GD-ODE $\dot X(t) = -\nabla f(X(t))$, which only achieves a rate $\OO(1/t)$.

A closer look at Tb.~\ref{tb:memories} reveals that the choice $3/t$ is related to \ref{MG-ODE} with quadratic forgetting, that is $\ddot X(t) +\frac{3}{t}\dot X(t) +\frac{3}{t} \nabla f(X(t))=0$. However, it is necessary to note that in \ref{MG-SDE} also the gradient term is premultiplied by $3/t$. Here we analyse the effects of this intriguing difference and its connection to acceleration.

% In this subsection we provide some new insights on this phenomenon and its interplay with uncertainty in gradient estimation.

\vspace{-2mm}
\paragraph{Gradient amplification.}
A na\"ive way to speed up the convergence of the GD-ODE $\dot X(t) = -\nabla f(X(t))$ is to consider $\dot X(t) = -t\nabla f(X(t))$. This can be seen by means of the Lyapunov function $\EE(x,t) = t^2(f(x)-f(x^*)) +\|x-x^*\|^2$. Using convexity of $f(\cdot)$, we have $\dot \EE(X(t),t) = -t^2\|\nabla f(X(t))\|^2\le 0 $ and therefore, the solution is s.t. $f(X(t))-f(x^*)\le \mathcal{O}(1/t^2)$. However, the Euler discretization of this ODE is the gradient-descent-like recursion $x_{k+1} = x_{k} -\eta k \nabla f(x_k)$ --- which is \textit{not} accelerated. Indeed, this \textit{gradient amplification} by a factor of $t$ is effectively changing the Lipschitz constant of the gradient field from $L$ to $kL$. Therefore, each step is going to yield a descent only if\footnote{See e.g. \cite{bottou2018optimization}.} $\eta \le \frac{1}{kL}$. Yet, this iteration dependent learning rate effectively cancels out the gradient amplification, which brings us back to the standard convergence rate $\mathcal{O}(1/k)$. It is thus natural to ask: "\textit{Is the mechanism of acceleration behind Nesterov's ODE related to a similar gradient amplification?}"


In App.~\ref{app:nesterov_vs_quadratic_noise} we show that $\{X_N(t), V_N(t)\}_{t\ge0}$, the solution to Nesterov's SDE\footnote{Nesterov's SDE is defined, as for \ref{MG-SDE} by augmenting the phase space representation with a volatility term. The resulting system is then : $dX(t) = V(t) dt; \  dV(t) = -3/t V(t) dt -\sigma(X(t))dB(t)$.}, is s.t. the infinitesimal update direction $V_N(t)$ of the position $X_N(t)$ can be written as
\begin{equation}
    V_{N}(t) =  -\int_0^t \frac{s^{3}}{t^3}\nabla f(X(s))ds  +\zeta_{N}(t),
    \label{eq:vn}
\end{equation}
where $\zeta_{N}(t)$ is a random vector with $\E[\zeta_{N}(t)]=0$ and $\var[\zeta_{N}(t)]=\frac{1}{7} t\sigma\sigma^T$. In contrast, the solution $\{X_{\m2}(t), V_{\m2}(t)\})_{t\ge 0}$ of \ref{MG-SDE} with quadratic forgetting satisfies
\begin{equation}
    V_{\m2}(t) =  -\int_0^t \frac{3s^{2}}{t^3}\nabla f(X(s))ds  +\zeta_{\m2}(t),
    \label{eq:vm}
\end{equation}

\begin{figure}
  \centering
    \includegraphics[width=0.97\linewidth]{img/unstable_nesterov.png} 
    \caption{\footnotesize{HB-SDE with $\alpha(t)=3/t$ (i.e. Nesterov's SDE) compared to \ref{MG-SDE} with quadratic forgetting. Setting as in \cite{su2014differential}: $f(x) = 2\times10^{-2} x_1^2 + 5\times10^{-3} x_2^2$ starting from $X_0 = (1,1)$ and $\dot X(0) = (0,0)$. Both systems are exposed to the same noise volatility. Simulation using the Milstein scheme \cite{mil1975approximate} with stepsize $10^{-3}$.}
    }
    \label{fig:HB_amplification}
\end{figure}


where $\zeta_{\m2}(t)$ is a random vector with $\E[\zeta_{\m2}(t)]=0$ but $\var[\zeta_{\m2}(t)]=\frac{9}{5t}\sigma\sigma^T$.
Even though the reader might already have spotted an important difference in the noise covariances, to make our connection to gradient amplification even clearer, we consider the simpler setting of constant gradients: in this case, we have $V_{N}(t) =  -\frac{1}{4} t \nabla f(X(t))  +\zeta_{N}(t)$, $V_{\m2}(t) =  -\nabla f(X(t))  +\zeta_{\m2}(t)$. That is, stochastic algorithms with increasing momentum (i.e. decreasing\footnote{See the connection between $\alpha$ and $\beta$ in Thm.~\ref{thm:HB_discretization}.} viscosity, like the Nesterov's SDE) \textit{are systematically amplifying the gradients over time}. Yet, at the same time they also linearly amplify the noise variance (see Fig.~\ref{fig:verif_noise} in the appendix). This argument can easily be extended to the non-constant gradient case by noticing that $\E[V_{\m2}(t)]$ is a weighted average of gradients where the weights integrate to 1 for all $t\ge 0$ (Lemma~\ref{lemma:unbiased}) . In contrast, in $\E[V_{N}(t)]$ these weights integrate to $t/4$. This behaviour is illustrated in Fig.~\ref{fig:HB_amplification}: While the Nesterov's SDE is faster compared to~\ref{MG-SDE} with $\m(t) = t^3$ at the beginning, it quickly becomes unstable because of the increasing noise in velocity and hence position. 

This gives multiple insights on the behavior of Nesterov's accelerated method for convex functions, both in for deterministic and the stochastic gradients:
\vspace{-3mm}
\begin{enumerate}
    \item Deterministic gradients get linearly amplified overtime, which counteracts the slow-down induced by the vanishing gradient problem around the solution. Interestingly Eq.~\eqref{eq:vn} reveals that  this amplification is \textit{not} performed directly on the local gradient but on past history, with \textit{cubic} forgetting. It is this feature that makes the discretization stable compared to the na\"ive approach $\dot X = -t\nabla f(X(t))$.
    \item Stochasticity corrupts the gradient amplification by an increasing noise variance (see Eq.~\eqref{eq:vn}), which makes Nesterov's SDE unstable and hence not converging. This finding is in line with~\cite{allen2017katyusha}.
\end{enumerate}
\vspace{-2mm}
Furthermore, our analysis also gives an intuition as to why a constant momentum cannot yield acceleration. Indeed, we saw already that \ref{HB-ODE-INT-C} does not allow such persistent amplification, but at most a constant amplification inversely proportional to the (constant) viscosity. Yet, as we are going to see in Sec.~\ref{sec:analysis_discretization}, this feature makes the algorithm more stable under stochastic gradients.

To conclude, we point the reader to App.~\ref{sec:quadratic_variance}, where we extend the last discussion from the constant gradient case to the quadratic cost case and get a close form for the (exploding) covariance of Nesterov's SDE (which backs up theoretically the unstable behavior shown in Fig.~\ref{fig:HB_amplification}). Nonetheless, we remind that this analysis still relies on continuous-time models; hence, the results above can only be considered as insights and further investigation is needed to translate them to the actual NAG algorithm.

\vspace{-2mm}
\paragraph{Time warping of linear memory.}
Next, we now turn our attention to the following question: "\textit{How is the gradient amplification mechanism of NAG related to its --- notoriously wiggling\footnote{Detailed simulations in App.~\ref{app:ODEs_quadratic}.}--- path?}". Even though Nesterov's ODE and \ref{MG-ODE} with quadratic forgetting are described by similar formulas, we see in Fig. \ref{fig:HB_amplification} that the trajectories are very different, even when the gradients are large. The object of this paragraph is to show that Nesterov's path has a strong link to --- surprisingly --- linear forgetting. Consider speeding-up the linear forgetting ODE $\ddot X(t) + \frac{2}{t} \dot X(t) + \frac{2}{t} \nabla f(X(t))$ by introducing the time change $\tau(t) = t^2/8$ and let $Y(t) = X(\tau(t))$ be the \textit{accelerated} solution to linear forgetting. By the chain rule, we have $\dot Y(t) = \dot\tau(t) \dot X(\tau(t))$ and $\ddot Y(t) = \ddot\tau(t) \dot X(\tau(t)) + \dot\tau(t)^2\ddot X(\tau(t))$.  It can easily be verified that we recover $\ddot Y(t) + \frac{3}{t} \dot Y(t) + \nabla f(Y(t))$. However, in the stochastic setting, the behaviour is still quite different: as predicted by the theory, in Fig. \ref{fig:timewarp} we see that --- when gradients are large --- the trajectory of the two sample paths are almost identical$^{11}$ (yet, notice that Nesterov moves faster); however, as we approach the solution, Nesterov diverges while linear forgetting stably proceeds towards the minimizer along the Nesterov's ODE path, but at a different speed, until convergence to a neighborhood of the solution, as proved in Sec.~\ref{sec:analysis_discretization}.
Furthermore, in App. \ref{time} we prove that there are no other time changes which can cast \ref{MG-ODE} into \ref{HB-ODE}, which yields the following interesting conclusion: the \textit{only} way to translate a memory system into a momentum method is by using a time change $\tau(t) = \mathcal{O}(t^2)$.
 
 \begin{figure}
  \centering
     \includegraphics[width=0.97\linewidth]{img/nesterov_timewarp.png}\caption{\footnotesize{Nesterov's ODE compared to \ref{MG-SDE} with linear forgetting (i.e. $\dot\m(t) / \m(t) = 2/t$). Same settings as Fig. \ref{fig:HB_amplification}.}}
    \label{fig:timewarp}
\end{figure}

\begin{table*}
\centering
\small{
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{| l | l | l | l |}
  \hline
  \textbf{Forgetting}& \textbf{Assumption} &  \textbf{Rate} &  \textbf{Reference} \\
  \hline
  Instantaneous & \textbf{(H0c)}, \textbf{(H1)}& $\E[f(\bar X(t))-f(x^*)] \le C_i / t  + \  d\ \sigma^2_*/2$& \cite{mertikopoulos2018convergence}\\   
  \hline
  Exponential & \textbf{(H0c)}, \textbf{(H1)}& $\E[f(\bar X(t))-f(x^*)] \le C_e / t  + \  d \ \sigma^2_*/2$& App. \ref{proofs}, Thm. \ref{prop:CONV_HBF_WQC_app}\\
  \hline
    Polynomial  & \textbf{(H0c)}, \textbf{(H1)}, $p\ge 2$& $\E[f(X(t))-f(x^*)] \le C_p/ t + p \  d \ \sigma^2_*/2$& App. \ref{proofs}, Thm. \ref{prop:memory_continuous_WQC}\\    
\hline
\end{tabular}
\egroup
}
\caption{\footnotesize{Rates of \ref{MG-SDE} on convex smooth functions . $\bar X(t)=\int_0^t X(s)ds$} and $C_i, C_e, C_p$ can be found in the references.}
\label{tb:summary_rates_cont}
\end{table*}

\section{ANALYSIS AND DISCRETIZATION}
\label{sec:analysis_discretization}
\vspace{-1mm}
In this section we first analyze the convergence properties of \ref{MG-SDE} under different memory functions. Next, we use the Lyapunov analysis carried out in continuous-time to derive an iterative discrete-time method which implements polynomial forgetting and has provable convergence guarantees. We state a few assumptions:

\textbf{(H0c)} $f\in\C^3_b(\R^d,\R), \ \sigma_*^2 := \sup_{x} \|\sigma(x)\sigma(x)^T\|_s < \infty$.

The definition of $\sigma_*^2$ nicely decouples the measure of noise magnitude to the problem dimension $d$ (which will then, of course, appear explicitly in all our rates).

\textbf{(H1)} \ \ The cost $f(\cdot)$ is $L$-smooth and convex.

\textbf{(H2)} \ \ The cost $f(\cdot)$ is $L$-smooth and $\mu$-strongly convex.

We provide the proofs (under the less restrictive assumptions of weak-quasi-convexity and quadratic growth\footnote{$\tau$-weak-quasiconvexity is implied by convexity and has been shown to be of chief importance in the context of learning dynamical systems~\cite{hardt2018gradient}. Strong convexity implies quadratic growth with a unique minimizer~\cite{karimi2016linear} as well as $\tau$-weak-quasiconvexity. More details in the appendix.}), as well as an introduction to stochastic calculus, in App.~\ref{proofs}.

\subsection{EXPONENTIAL FORGETTING}
If $\m(t) = e^{\alpha t}-1$, then $\dot\m(t)/\m(t) = \frac{\alpha e^{\alpha t}}{e^{\alpha t}-1}$ which converges to $\alpha$ exponentially fast. To simplify the analysis and for comparison with the literature on HB-SDE~(which is usually analyzed under constant volatility \cite{shi2018understanding}) we consider here \ref{MG-SDE} with the approximation $\dot\m(t)/\m(t)\simeq\alpha$. In App.~\ref{proofs} we show that, under \textbf{(H1)}, the rate of convergence of $f(\cdot)$, evaluated at the Cesàro average $\bar X(t) = \int_0^t X(s)ds$ is sublinear~(see Tb. \ref{tb:summary_rates_cont}) to a ball\footnote{Note that the term "ball" might be misleading: indeed, the set $\mathcal{N}_\epsilon(x^*) = \{x\in\R^d, f(x)-f(x^*)\le\epsilon\}$ is not compact in general if $f(\cdot)$ is convex but not strongly convex.} around $x^*$ of size $d \ \sigma^2_*/2$, which is in line with known results for SGD \cite{bottou2018optimization}\footnote{Note that, by definition of $\sigma(\cdot)$ (see discussion after \ref{MG-SDE}), $\sigma^2_*$ is proportional both to the learning rate and to the largest eigenvalue of the stochastic gradient covariance}. Note that the size of this ball would change if we were to study a stochastic version of~\ref{HB-ODE} with constant volatility (i.e. $\ddot X + \alpha \dot X + \nabla f(X)$). In particular, it would depend on the normalization constant in  Eq.~\eqref{normalization_step}.  Also, in App.~\ref{proofs}, under \textbf{(H2)}, we provide a \textit{linear} convergence rate of the form $f(X(t))-f(x^*)\le \mathcal{O}(e^{-\gamma t})$ to a ball ($\gamma$ depends on $\mu$ and $\alpha$). Our result generalizes the analysis in \cite{shi2018understanding} to work with \textit{any viscosity} and with stochastic gradients. 

\vspace{-2mm}
\paragraph{Discretization.} As shown in Sec.~\ref{sec:mem_fun_grad_forg}, the discrete equivalent of~\ref{MG-SDE} with exponential forgetting is Adam without adaptive stepsizes (see App.~\ref{sec:unbiasing}). As for the continuous-time model we just studied, for a sufficiently large iteration, exponential forgetting can be approximated with the following recursive formula:
 $$x_{k+1} = x_k + \beta (x_k-x_{k-1}) - \eta(1-\beta)\nabla f(x_k),$$
which is exactly \ref{HB} with learning rate $(1-\beta)\eta$. Hence, the corresponding rates can be derived from Tb.~\ref{tb:summary_existing_rates}.  

\subsection{POLYNOMIAL FORGETTING}
The insights revealed in Sec.~\ref{nesterov_comparison} highlight the  importance of the choice $\m(t) = t^p$ in this paper. In contrast to instantaneous~\cite{mertikopoulos2018convergence} and exponential forgetting, the rate we prove in App.~\ref{proofs} for this case under \textbf{(H1)} does not involve a Cesàro average --- \textit{but holds for the last time point} (see Tb.~\ref{tb:summary_rates_cont}). This stability property is directly linked to our discussion in Sec.~\ref{nesterov_comparison} and shows that different types of memory may react to noise very differently. Also, we note that the size of the ball we found is now also proportional to $p$; this is not surprising since, as the memory becomes more focused on recent past, we get back to the discussion in the previous subsection and we need to consider a Cesàro average.
\vspace{-2mm}
\paragraph{Discretization.} Finally, we consider the burning question "\textit{Is it possible to discretize~\ref{MG-SDE} --- with polynomial forgetting --- to derive a cheap iterative algorithm with similar properties?}". In App.~\ref{poly-discre}, we build this algorithm in a non-standard way: we  reverse-engineer the proof of the rate for~\ref{MG-SDE} to get a method which is able to mimic each step of the proof. Starting from $x_{-1} = x_0$, it is described by the following recursion

\begin{tcolorbox}
\vspace{-5mm}
\begin{equation}
    \tag{MemSGD-p}
    x_{k+1} = x_k + \frac{k}{k+p} (x_k-x_{k-1}) - \frac{p}{k+p} \eta \nabla f(x_k).
    \label{MemSGD-p}
\end{equation}
\vspace{-5mm}
\end{tcolorbox}

As a direct result of our derivation, we show in Thm.~\ref{thm:discretization} (App.~\ref{poly-discre}) that \textit{this algorithm preserves exactly the rate} of its continuous-time model in the stochastic setting\footnote{Required assumptions: \textbf{(H1)}, $p\ge 2$, $\eta\le \frac{p-1}{pL}$ and $\varsigma_*^2$ bounds the gradient variance in each direction of $\R^d$.}:
$$\E[f(x_k)-f(x^*)] \le \frac{(p-1)^2\|x_0-x^*\|^2}{2 \eta p (k+p-1)} + \frac{1}{2}p d \eta \varsigma_*^2 .$$
We also show that \ref{MemSGD-p} can be written as $x_{k+1} = x_k -\eta\sum_{j=0}^k w(j,k)\nabla f(x_k)$, where $\sum_{j=0}^k w(j,k)=1$ (in analogy to the bias correction in Adam) and with $ w(\cdot,k)$ increasing as a polynomial of order $p-1$ for all $k$, again in complete analogy with the model. Fig.~\ref{fig:p_verification} shows the behaviour of different types of memory in a simple convex setting; as predicted, polynomial (in this case linear) forgetting has a much smoother trajectory then both exponential and instantaneous forgetting. Also, the reader can verify that the asymptotic noise level for MemSGD (p=2) is slightly higher, as just discussed. 

For ease of comparison with polynomial memory, we will often write MemSGD (p=e) to denote exponential forgetting (i.e. Adam without adaptive steps) and SGD (p=inf) to stress that SGD implements instantaneous forgetting.


 \begin{figure}
  \centering
    \includegraphics[width=0.65\linewidth]{img/p-verification2}\caption{\footnotesize{Synthetic example: $f(x_1,x_2) = 0.8\times x_1^4 + 0.4\times x_2^4$ with Gaussian noise. Displayed is linear forgetting (i.e. MemSGD-2), exponential forgetting (denoted p=e) with $\beta = 0.8$ and instantaneous forgetting. Average and 95\% confidence interval for 150 runs starting from $(1,1)$.}}
    \label{fig:p_verification}
\end{figure}

